Invariance Through Latent Alignment

A robot's deployment environment often involves perceptual changes that differ from what it has experienced during training. Standard practices such as data augmentation attempt to bridge this gap by augmenting source images in an effort to extend the support of the training distribution to better cover what the agent might experience at test time. In many cases, however, it is impossible to know test-time distribution-shift a priori, making these schemes infeasible. In this paper, we introduce a general approach, called Invariance Through Latent Alignment (ILA), that improves the test-time performance of a visuomotor control policy in deployment environments with unknown perceptual variations. ILA performs unsupervised adaptation at deployment-time by matching the distribution of latent features on the target domain to the agent's prior experience, without relying on paired data. Although simple, we show that this idea leads to surprising improvements on a variety of challenging adaptation scenarios, including changes in lighting conditions, the content in the scene, and camera poses. We present results on calibrated control benchmarks in simulation -- the distractor control suite -- and a physical robot under a sim-to-real setup.

==> results/original_table.tex <==
\begin{table}[ht]
\centering
\caption{Ablation studies}
\label{table:ablation}
\begin{tabularx}{\linewidth}{Xccc}
\toprule
Distraction & w/o inv.\ dynamics & w/o adv.\ training & Inv thru Inf\\
\midrule
Camera       & $\bm{741.29 \pm 280.22}$  & $292.46 \pm 385.33$     & $674.20 \pm 259.02$ \\
Background   & $\bm{715.43 \pm 303.36}$  & $199.97 \pm 283.93$     & $655.03 \pm 327.19$ \\
Color        & $\bm{728.42 \pm 311.81}$  & $239.05 \pm 310.65$     & $682.51 \pm 342.29$ \\
% Average      & 0  & 0     & 0 \\ % I'll do this if I got time --- takuma
\bottomrule
\end{tabularx}
\end{table}

==> sections/closing_remarks.tex <==
\section{Closing Remarks}
%

\begin{table}[t]
    \centering
    \caption{Comparison with PAD}
    \begin{tabularx}{0.8\linewidth}{Xcccc}
    \toprule
    % & \multicolumn{2}{c}{\makebox[0pt]{Before Adaptation}} & \multicolumn{2}{c}{\makebox[0pt]{After Adaptation}}\\
    Distraction & Zero-shot & +PAD & +ILA\\
    \midrule
    
    None          & $835^{\scriptscriptstyle\pm 230} $ & ---  & --- \\ 
    Background    & $213^{\scriptscriptstyle\pm 247} $ & $ 279^{\scriptscriptstyle\pm 271}$ & $ \bm{425^{\scriptscriptstyle\pm 292}}$ \\
    Colors        & $230^{\scriptscriptstyle\pm 263}$ & $ 271^{\scriptscriptstyle\pm 300}$ & $ \bm{402^{\scriptscriptstyle\pm 339}}$ \\
    Camera Pose   & $319^{\scriptscriptstyle\pm 265}$ & $ 326^{\scriptscriptstyle\pm 259}$ & $ \bm{412^{\scriptscriptstyle\pm 275}}$ \\
    \bottomrule
    \end{tabularx}
    \label{table:pad}
\end{table}
%

We introduced \textit{\lcila}, an unsupervised approach that matches the distribution of feature vectors in the latent space, to improve the test-time performance of a learned visuomotor control policy. Empirical results demonstrate that as discrepancies between the training and deployment environments become more intense, \lcila has a large competitive edge over alternatives such as data augmentation techniques. The problem of test-time adaptation in visual reinforcement learning using unsupervised test-time trajectories is relatively new, but has thus far shown great relevance and promise in robotics~\cite{hansen2020pad,hansen2021soda}, where a sim-to-real pipeline has been at the fore-front of recent progress~\cite{Kaufmann2018drone,Wu2019deformable,margonlis2022rapid}.

A problem that remains is sampling. Technically, the distribution of trajectories and their latent representation on the source domain depends on the policy. There are state transitions that are only accessible through a performant policy. To our surprise, a simple scheme that uses the random policy to collect data on both the source and the target domain largely by-passes this issue and is able to achieve good performance post-adaptation. Future work in this area might want to develop better techniques for data generation at test time, so that the collected trajectory data better resembles those collected by the agent in the source buffer. One version of the scheme resembles generative adversarial imitation learning (GAIL, see~\cite{Ho2016gail}). Another open problem is that the performance does not improve monotonically upon more unsupervised updates. Finding an improvement scheme that is provably monotonic would be interesting. Finally, although the adversarial distribution matching objective proposed here produce measurable improvements, better schemes for feature alignment are still needed. For a recent work in this direction, we refer the reader to \textit{adversarial support alignment}~\cite{tong2022support}.

\section{Acknowledgements}

This work was funded in part by the National Science Foundation under grant IIS-1830660. Ge Yang is supported by the National Science Foundation Institute for Artificial Intelligence and Fundamental Interactions (IAIFI, \href{https://iaifi.org/}{https://iaifi.org/}) under the Cooperative Agreement PHY-2019786. The authors would like to thank Adam Bohlander and Greg Shakhnarovich at the Toyota Technological Institute at Chicago (TTIC) for computing resources and additional storage. This paper also benefited from thoughtful discussions with students in the TTIC robotics group. The authors would also like to acknowledge the MIT SuperCloud and Lincoln Laboratory Supercomputing Center for providing high performance computing resources.


==> sections/experiments.tex <==
\section{Experiments}



%\stadie{Finished editing. Ready for feedback and another pass @Ge, @Takuma October 5, 01:03am}

\label{sec:experiments}
% Motivation: Invariance through Memorization degrades in performance when the variance becomes larger
% whereas our method does not.
% \paragraph{Setup} Provide an outline of the experiments, and summarize the results
% Introduce the domains, a screenshot of different types of distractions
%\takuma{ (About the first sentence) Should we say "compare our method against" other method or "apply our method on top of " theirs?}

%Our primary focus in this section will be understanding the 

\begin{table*}[h!]
\centering
\caption{Episode return in the target (test) environments (mean and standard deviation) before (zero-shot) and after (+ILA) adaptation for SAC, SVEA, and DrQ-v2 with background distraction at an intensity setting of $1.0$. The performance of each baseline in the source (training) environments can be found in the Appendix.}\label{table:baseline-adaptation}{\small%
\setlength{\tabcolsep}{8pt}
\begin{tabularx}{0.8\linewidth}{Xcc|cc|cc}
    \toprule
                       & \multicolumn{2}{c}{SAC}                                          & \multicolumn{2}{c}{SVEA}                                                       & \multicolumn{2}{c}{DrQ-v2}\\
    Domain              & Zero-shot                 & +ILA                                  & Zero-shot                             & +ILA                                  & Zero-shot                     & +ILA \\
    \midrule
\texttt{ball\_in\_cup-catch} & $115^{\scriptscriptstyle\pm 50} \hphantom{0}$  & $\bm{227^{\scriptscriptstyle\pm 222}}$              & $490^{\scriptscriptstyle\pm 376}$                          & $\bm{987^{\scriptscriptstyle\pm 27}} \hphantom{0}$    & $\hphantom{0}88^{\scriptscriptstyle\pm 39} \hphantom{0}$     & $\bm{386^{\scriptscriptstyle\pm 425}}$    \\
\texttt{cartpole-balance}    & $434^{\scriptscriptstyle\pm 275}$             & $\bm{585^{\scriptscriptstyle\pm 295}}$              & $446^{\scriptscriptstyle\pm 330}$                          & $\bm{627^{\scriptscriptstyle\pm 258}}$               & $273^{\scriptscriptstyle\pm 107}$                           & $\bm{322^{\scriptscriptstyle\pm 117}}$    \\
\texttt{cartpole-swingup}    & $182^{\scriptscriptstyle\pm 147}$             & $\bm{369^{\scriptscriptstyle\pm 243}}$              & $269^{\scriptscriptstyle\pm 365}$                          & $\bm{612^{\scriptscriptstyle\pm 213}}$               & $\hphantom{0}82^{\scriptscriptstyle\pm 35}\hphantom{0}$     & $\bm{247^{\scriptscriptstyle\pm 136}}$    \\
\texttt{cheetah-run}         & $169^{\scriptscriptstyle\pm 65} \hphantom{0}$  & $\bm{248^{\scriptscriptstyle\pm 53}}\hphantom{0}$   & $317^{\scriptscriptstyle\pm 137}$                          &  $\bm{378^{\scriptscriptstyle\pm 55}}\hphantom{0}$    & $100^{\scriptscriptstyle\pm 88}\hphantom{0}$                & $\bm{393^{\scriptscriptstyle\pm 125}}$    \\
\texttt{finger-spin}         & $113^{\scriptscriptstyle\pm 162}$             & $\bm{192^{\scriptscriptstyle\pm 196}}$              & $391^{\scriptscriptstyle\pm 467}$                          & $\bm{943^{\scriptscriptstyle\pm 54}}\hphantom{0}$    & $207^{\scriptscriptstyle\pm 328}$                           & $\bm{769^{\scriptscriptstyle\pm 206}}$    \\
\texttt{finger-turn\_easy}   & $\bm{163^{\scriptscriptstyle\pm 99}}\hphantom{0}$  & $146^{\scriptscriptstyle\pm 33} \hphantom{0}$   & $278^{\scriptscriptstyle\pm 180}$                          & $\bm{491^{\scriptscriptstyle\pm 343}}$  &  $268^{\scriptscriptstyle\pm 241}$   & $\bm{914^{\scriptscriptstyle\pm 44}}\hphantom{0}$  \\
\texttt{reacher-easy}        & $179^{\scriptscriptstyle\pm 65}\hphantom{0}$  & $\bm{381^{\scriptscriptstyle\pm 76}}\hphantom{0}$   & $\hphantom{0}75^{\scriptscriptstyle\pm 77} \hphantom{0}$    & $\bm{624^{\scriptscriptstyle\pm 305}}$               & $\hphantom{0}58^{\scriptscriptstyle\pm 32}\hphantom{0}$     & $\bm{685^{\scriptscriptstyle\pm 211}}$    \\
\texttt{walker-stand}        & $330^{\scriptscriptstyle\pm 118}$             & $\bm{364^{\scriptscriptstyle\pm 115}}$              & $917^{\scriptscriptstyle\pm 138}$                          & $\bm{999^{\scriptscriptstyle\pm 12}} \hphantom{0}$    & $630^{\scriptscriptstyle\pm 197}$                           & $\bm{868^{\scriptscriptstyle\pm 151}}$    \\
\texttt{walker-walk}         & $242^{\scriptscriptstyle\pm 142}$             & $\bm{291^{\scriptscriptstyle\pm 134}}$              & $866^{\scriptscriptstyle\pm 45}\hphantom{0}$               & $\bm{924^{\scriptscriptstyle\pm 45}}\hphantom{0}$    & $326^{\scriptscriptstyle\pm 195}$                           & $\bm{770^{\scriptscriptstyle\pm 140}}$ \\  
    \bottomrule
\end{tabularx}}
\end{table*}

We want to understand the impact of test-time inference on an agent's ability to generalize out-of-distribution. This section will compare \ac{ILA} with two state-of-the-art reinforcement learning baselines that uses data-augmentation: SVEA~\citep{svea} and DrQ-v2~\citep{yarats2021drqv2}. %\todoty{I will most likely include SODA as well.} \todomw{This is something that we should discuss}    
Recall from the introduction that these methods vie for increased generalization capabilities by expanding the support of the training distribution. We expect the invariance produced this way to be less performant than unsupervised adaptation at test time that only needs to focus on one specific instance of perceptual variation. In our experiments, we will also compare against \textit{policy adaptation during deployment} (PAD, see~\citep{hansen2020pad}), a baseline that, like our method, adapts the policy without access to the reward at test time. 

%Unsupervised adaptation in the context of deep reinforcement learning is a relatively new area. To date, the primary baseline has been Policy Adaptation During Deployment (PAD)~\citep{padhansen2020selfp}. Similar to our approach, PAD pre-trains the agent in a clean environment, and then adapts the agent via unsupervised transfer, without assuming access to the target environment's reward function. PAD itself proceeds by pre-training an agent with an auxiliary inverse dynamics task, and then using this prediction head to guide an encoder during the adaption phase.\todomw{This paragraph is a bit redundant given the discussion of PAD in the first paragraph of the results section.}
To further probe the generalization abilities of test-time inference, we conduct an experiment where we vary the intensity of environmental distractions. The results show that test-time inference significantly increases the policy performance during deployment. We will conclude with some general discussion and remarks regarding the design tradeoffs involved in test-time inference.  


%We also compare against 




%We compare our method to contemporary methods that employ data augmentation to encourage generalizability, specifically SVEA~\citep{} and DrQv2~\citep{}.
%We first compare our adaptation scheme, \textit{invariance through inference}, against methods that adopt data-augmentation regime where they attempt to cover a broad distributions at training time. We make comparisons with state-of-the-art methods in this domain, including SVEA \citep{} and DrQv2 \citep{}, and show that our method can provide better test-time performance in highly distracting environments. 
%We then evaluate the extent to which our approach generalizes to test-time variations by varying the \textit{intensity} of distractions, and show that the episode return deteriorates comparably slower with our approach as distraction intensity increases while consistently presenting a better performance.
% I keep saying "compare" what's the alternative phrasing?
%We also compare against Policy Adaptation during Deployment (PAD)~\citep{padhansen2020selfp}, which similarly adapts the policy without access to the reward at test time.

%We now compare our method, \textit{invariance through inference}, against methods that try to ``bake-in'' the sense of invariance at training time, on test-time distribution that are out of the training distribution. We compare against state-of-the-art methods in this domain including SODA and SVEA, in addition to PAD which also uses self-supervised adaptation objective after deployment. We evaluate all approaches on variants of the distracting control suite~\citep{stone}.

% Setup is too long....
\paragraph{Setup} We conduct experiments on nine domains from the DeepMind Control Suite (DMC, see~\citep{deepmindcontrolsuite2018}) and treat it as the \textit{source} domain for training the RL agents. We use the Distracting Control Suite ~\citep{stone2021distracting} as the \textit{target} domain. Distracting control suite adds three types of distractions to DMC, including image background, random color texture, and changes to the camera pose. The intensity of these modes of distraction are calibrated. For details, refer to the accompanying report (see~\citealt{stone2021distracting})

\paragraph{Modifications to Distracting Control Suite}
The default configuration of distracting control suite changes distractions at the start of every episode (e.g., different background images are used at every episode). However, we are interested in measuring an agent's ability to perform inference across several episodes on the same target environment. Thus, we modify distracting control suite to sample a distraction once in the beginning of learning, and then use the same distraction across all learning epochs. This also ensures consistent evaluation across algorithms. In accordance with this change, we also modify the intensity benchmark from distracting control suite. In our experiments, intensity measures the deviation between an environment distraction and the train environment's default value. For example, intensity may measure how far the distracting color is from the default. Finally, we modify the environments to only apply a single distraction during testing (rather than all three) in order to better understand the impact of each type of distraction on overall performance. Figure~\ref{fig:distractions} shows an example of distractions across intensities on Walker-walk domain.

Table~\ref{table:baseline-adaptation} presents the results for the different distracting control suite domains in the presence of background distractions with an intensity level of $1.0$. Specifically, we compare the test-time performance of SAC, SVEA, and DrQ-v2 in each domain with the episode rewards that we achieve when using \ac{ILA} algorithm to adapt the encoder. The baseline algorithms employ image augmentation, which provides some robustness to variations at test time. Even then, however, we find that \ac{ILA} adaptation improves the test-time generalization of all three baseline policies in most domains, often resulting in significant performance gains. In cases where \ac{ILA} does not improve performance, the resulting reward is comparable to the baseline policy, i.e., \ac{ILA} does not result in a performance degradation.

Figure~\ref{fig:intensity-vs-reward} visualizes the performance of the different methods, averaged over the set of distracting control suite domains, as a function of the intensity of the distractions. Since the baseline methods are trained with image augmentation, they do exhibit some robustness to distraction. However, we see this robustness rapidly diminishes as the distraction intensity increases. In particular, large changes to camera pose or the image background proved challenging for standard augmentation procedures. Comparatively, \ac{ILA} makes it much smoother and slower degradation of performance. This supports our hypothesis that adaptation powered by unsupervised learning can significantly widen the generalization abilities of learning algorithms.%\todomw{A fairly broad hypthesis}


%In this setting background image, for example, changes only when a different random seed is used.  % Takuma --- The last sentence may be rather confusing ?
%Accordingly, we alter the definition of \textit{intensity} to be the departure from the default value (i.e., how far the distracting color is from the default), rather than the width of distribution (e.g., how large the distraction sample space is) as in distracting control suite.
%Finally, we modified it to apply only one of the distraction types. This enables us to understand what effect a type of distraction does to performance.


\subsection{\ac{ILA} on DeepMind Control Suite}


%

% Key Experiments
% What are the axis: mode, scale, 
% \paragraph{Invariance over larger range} 
% sweep over the parameters and show better robustness because train on test allows us to overfit to a particular deployment instance. Compare against PAD, SODA, SVEA, DrQ etc.

% Takuma
%Our goal here is to understand how well our method improves performance in the out-of-distribution distracting environment.
This section studies the impact of test-time adaptation on DeepMind control suite performance. We begin by pretraining soft actor-critic (SAC)~\citep{sacapps}, SVEA, and DrQ-v2 in a non-distracting training-time environment. After training, we evaluate the learned policies on test environments with distractions of various intensities. This evaluation is zero-shot, i.e., there is no additional training in the test environment. 

%This is expected, as pre-defined augmentations cannot cover the entire distraction distribution, espe


%such as camera pose distraction or unseen image background.



%The plots can be found in Fig. %\ref{fig:intensity-vs-reward}.
%All methods except for SAC are trained with image augmentation, and thus are expected to generalize to some extent. However, we observe that the performance drastically drops as distracting intensity increases. We believe this is because the pre-defined augmentations cannot cover the entire distraction distribution such as camera pose distraction or unseen image background.

%On top of these baseline methods, we applied our \textit{invariance-through-inference} adaptation on each target environment.
% To visualize how much gain we can obtain, we applied our \textit{invariance-through-inference} adaptation on top of each pre-trained agent.
%As can be seen in Fig. \ref{fig:intensity-vs-reward}, applying our method improves the performance. Notably, the episode return decays much slower with our method as its distraction intensity increases. This aligns with the intuition that adaptation with unsupervised learning can work with a wider range of out-of-distribution environments compared to those methods that attempt to learn a policy that can work with a wide range of distributions via augmentations.

%\takuma{I will add some observations about the plot here}

%\todointy{This table is ugly. Probably will ask Nick Hansen to provide his latex code to generate his nice table on SODA paper.}
%\todoinmw{I put a copy of the SVEA+SODA table that was here in the appendix}


% \begin{table}
% \caption{Episodic return in test environments with randomized colors, mean and std. dev. for 10 seeds. Best method on each task is in bold and blue compares SAC+IDM with and without PAD.\takuma{Numbers will be updated!!!}}
% \vspace{-0.05in}
% \label{tab:dmc-colors}
% \centering
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{lcc|cc|cc|cc}
% \toprule
% Background & \multicolumn{2}{c}{SVEA}                                          & \multicolumn{2}{c}{SAC} 
%           & \multicolumn{2}{c}{DrQ-v2}
%           & \multicolumn{2}{c}{SODA}  \\
%               & Zero-shot   & +ITI & Zero-shot   & +ITI      & Zero-shot   & +ITI     & Zero-shot   &  +ITI             \\
% \midrule

% ball\_in\_cup-catch & $490 \scriptstyle{ \pm 376 }$ & $987 \scriptstyle{ \pm 27\hphantom{0} }$  & $757 \scriptstyle{ \pm 308 }$ & $870 \scriptstyle{ \pm 176 }$ & $115 \scriptstyle{ \pm 50 }$  & $227 \scriptstyle{ \pm 222 }$ & $88 \scriptstyle{ \pm 39 }$   & $386 \scriptstyle{ \pm 425 }$ \\
% cartpole-balance    & $446 \scriptstyle{ \pm 330 }$ & $627 \scriptstyle{ \pm 258 }$ & $941 \scriptstyle{ \pm 136 }$ & $865 \scriptstyle{ \pm 165 }$ & $434 \scriptstyle{ \pm 275 }$ & $585 \scriptstyle{ \pm 295 }$ & $273 \scriptstyle{ \pm 107 }$ & $322 \scriptstyle{ \pm 117 }$ \\
% cartpole-swingup    & $269 \scriptstyle{ \pm 365 }$ & $612 \scriptstyle{ \pm 213 }$ & $602 \scriptstyle{ \pm 140 }$ & $598 \scriptstyle{ \pm 151 }$ & $182 \scriptstyle{ \pm 147 }$ & $369 \scriptstyle{ \pm 243 }$ & $82 \scriptstyle{ \pm 35 }$   & $247 \scriptstyle{ \pm 136 }$ \\
% cheetah-run         & $317 \scriptstyle{ \pm 137 }$ & $378 \scriptstyle{ \pm 55 }$  & $121 \scriptstyle{ \pm 68 }$  & $148 \scriptstyle{ \pm 86 }$  & $169 \scriptstyle{ \pm 65 }$  & $248 \scriptstyle{ \pm 53 }$  & $100 \scriptstyle{ \pm 88 }$  & $393 \scriptstyle{ \pm 125 }$ \\
% finger-spin         & $391 \scriptstyle{ \pm 467 }$ & $943 \scriptstyle{ \pm 54 }$  & $581 \scriptstyle{ \pm 303 }$ & $623 \scriptstyle{ \pm 256 }$ & $113 \scriptstyle{ \pm 162 }$ & $192 \scriptstyle{ \pm 196 }$ & $207 \scriptstyle{ \pm 328 }$ & $769 \scriptstyle{ \pm 206 }$ \\
% finger-turn\_easy   & $278 \scriptstyle{ \pm 180 }$ & $491 \scriptstyle{ \pm 343 }$ & $501 \scriptstyle{ \pm 213 }$ & $628 \scriptstyle{ \pm 125 }$ & $163 \scriptstyle{ \pm 99 }$  & $146 \scriptstyle{ \pm 33 }$  &                               &                               \\
% reacher-easy        & $75 \scriptstyle{ \pm 77 }$   & $624 \scriptstyle{ \pm 305 }$ & $645 \scriptstyle{ \pm 286 }$ & $721 \scriptstyle{ \pm 308 }$ & $179 \scriptstyle{ \pm 65 }$  & $381 \scriptstyle{ \pm 76 }$  & $58 \scriptstyle{ \pm 32 }$   & $685 \scriptstyle{ \pm 211 }$ \\
% walker-stand        & $917 \scriptstyle{ \pm 138 }$ & $999 \scriptstyle{ \pm 12 }$  & $821 \scriptstyle{ \pm 379 }$ & $827 \scriptstyle{ \pm 361 }$ & $330 \scriptstyle{ \pm 118 }$ & $364 \scriptstyle{ \pm 115 }$ & $630 \scriptstyle{ \pm 197 }$ & $868 \scriptstyle{ \pm 151 }$ \\
% walker-walk         & $866 \scriptstyle{ \pm 45 }$  & $924 \scriptstyle{ \pm 45 }$  & $662 \scriptstyle{ \pm 54 }$  & $699 \scriptstyle{ \pm 88 }$  & $242 \scriptstyle{ \pm 142 }$ & $291 \scriptstyle{ \pm 134 }$ & $326 \scriptstyle{ \pm 195 }$ & $770 \scriptstyle{ \pm 140 }$ \\

\begin{figure}[b!]
    % \centering
    \begin{subfigure}[t]{0.35\linewidth}
        \includegraphics[height=70px]{results/learning-curve-20220505-noticklabels/color.pdf}
        \caption{Color}% \label{fig:adaptation-curves-colors}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.3\linewidth}
        \includegraphics[height=67.5px]{results/learning-curve-20220505-noticklabels/background.pdf}
        \caption{Background}% \label{fig:adaptation-curves-background}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.3\linewidth}
    \includegraphics[height=67.5px]{results/learning-curve-20220505-noticklabels/camera.pdf}
    \caption{Camera Pose}% \label{fig:adaptation-curves-camera}
  \end{subfigure}\hfill
    \caption{Relative improvement (compared to zero-shot) as a function of adaptation steps when applying ILA to different baseline policies. As in Figure~\ref{fig:intensity-vs-reward}, each point represents the mean over nine domains and five random seeds. The results correspond to a distraction intensity value of $1$.}
    \label{fig:adaptation-curves}
\end{figure}



% \begin{figure}[]
%     \centering
%     \hspace{-10px}
%   \begin{subfigure}[t]{0.3\linewidth}
%     \includegraphics[height=78px]{results/learning_curve-dotted-lines/background.pdf}
%     \caption{Background}% \label{fig:adaptation-curves-background}
%   \end{subfigure}\hfill
%   \begin{subfigure}[t]{0.3\linewidth}
%     \includegraphics[height=78px]{results/learning_curve-dotted-lines/color.pdf}
%     \caption{Colors}% \label{fig:adaptation-curves-colors}
%   \end{subfigure}\hfill
%   \begin{subfigure}[t]{0.3\linewidth}
%     \includegraphics[height=78px]{results/learning_curve-dotted-lines/camera.pdf}
%     \caption{Camera Pose}% \label{fig:adaptation-curves-camera}
%   \end{subfigure}
% %     \begin{subfigure}[t]{0.08\textwidth}
% %     \centering
% %     \includegraphics[trim={0px 12px 17px 5px}, clip, width=0.8\textwidth]{results/learning_curve/legend.pdf}
% %   \end{subfigure}\hfill
%     \caption{Relative improvement (compared to zero-shot) as a function of adaptation steps when applying ITI to different baseline policies. As in Figure~\ref{fig:intensity-vs-reward}, each point represents the mean over nine domains and five random seeds. The results correspond to a distraction intensity value of 1.0.}
%     \label{fig:adaptation-curves}
% \end{figure}

\subsection{Comparisons with PAD}
%\takuma{Need a better title}
%\stadie{Comparison with PAD is probably fine}
Similar to our approach, PAD pretrains the agent in a clean environment, and then adapts the agent via unsupervised objectives without assuming access to the target environment's reward function~\citep{hansen2020pad}. To evaluate the robustness of PAD to distractions, we consider distracting control suite with a fixed distraction intensity of $1.0$. Table~\ref{table:pad} compares the performance as the difference between the episode returns before and after adaptation along with the episode returns in the clean environment. It should be noted that PAD requires to pretrain a policy along with inverse dynamics prediction objective. Thus we trained SAC with the auxiliary objective specifically for this experiment.
% \todomw{Currently, Table 1 doesn't show percentage improvement} 
% i.e., $ \frac{r_\textrm{pre} - r_\textrm{post}}{r_\textrm{clean}}$, where $r_\textrm{pre}$ is the reward the agent obtains before adaptation, $r_\textrm{post}$ is the reward after adaptation, and $r_\textrm{clean}$ is the return on the corresponding clean environment. 

Across all environments, we see that PAD struggles to adapt to distractions at test time. We suspect this instability is caused by the large deviations in the latent variable distribution as a result of changes in the target environment. In particular, we posit that the signal from PAD's inverse dynamics head does not encourage the latent train and test distributions to match, whereas in \ac{ILA}, it does.
%PAD pre-trains an agent with auxiliary inverse dynamics task, and use its prediction head to guide the encoder during adaptation.



%For this experiment, we take intensity $0.6$ of each distraction type and evaluated the performances before and after adaptation. 



%Table \ref{table:x} shows our approach outperforms PAD across all distraction types. The percentage shows the gains normalized by its corresponding episode return in the clean environment. % We should separately train a policy directly on distracting environment and calculate this after submission.


%We consider that this is because the policy trained with latent distribution in the source environment cannot work well with the largely deviated latent distribution during target environment.
%The signals from the inverse dynamics head does not necessarily encourage these distributions to match, whereas our approach has the adversarial structure that encourages it.
% The policy trained with latent distribution during pre-training cannot work well with the largely deviated latent distribution during deployment.

% \begin{table}[ht]
% \centering
% \caption{Comparison against PAD}
% \begin{tabularx}{\linewidth}{Xcccccc}
% \toprule
% Distraction & SAC with InvD & PAD & \% & DrQv2 & Inv thru Inf & \% \\
% \midrule
% Camera       & 0             & 0   & 0  & 0     & 0                            & 0  \\
% Background   & 0             & 0   & 0  & 0     & 0                            & 0  \\
% Color        & 0             & 0   & 0  & 0     & 0                            & 0  \\
% Average      & 0             & 0   & 0  & 0     & 0                            & 0 \\
% \bottomrule
% \end{tabularx}
% \end{table}






% Takuma --- I'm not really sure about this:
%\paragraph{Interaction with Data Augmentation} sweep over different amount of data augmentation when combined with DrQ/SODA/SVEA. See if adding our additional objective helps with running on those methods.

% Main figures 

\subsection{Sim-to-real Transfer}
We are interested in the ability of \ac{ILA} to bridge the gap between simulated and real world robotics environments. In the {\it reaching} task, the target position is given by a red disc placed on a table. The agent's objective is to controls the arm so that the end-effector reaches this target location. Our goal is to train a policy in simulation, and then transfer the policy to a real UR-5 robot at test time. The same as with previous experiments, the test time agent receives no rewards. In both simulation and the real world, the policy's only input is an image from a camera placed in front of the robot and table. The action space is a 2D position controller that drives a small movement $(\delta x, \delta y)$ of the robotic gripper. See Figure~\ref{fig:sim2real} for the setup. 
%The front-view image \todoty{Does this wording make sense?} is used as an input to the policy, and the action space is 2D that moves the gripper's tip location on the table.

We carry out the experiment by first training a policy with SVEA~\cite{svea} in simulation. For adaptation, we collect random trajectories in the real environment and then use \ac{ILA} to align the simulated and real world experiences. We evaluated the success rate of zero-shot and the adapted policies over 20 real episodes. We consider the episode to be success if the gripper's tip overlaps with the target in the front-view image.

Due to the challenging domain shift between simulator and real world, the zero-shot policy fails to adapt adequately, repeating the same action of moving the gripper to an edge of the table ad infinitum, regardless of the given goal location. This results in a final success rate of 15\%. %, which is little better than random noise. 
On the same task, \ac{ILA} is able to robustly handle this domain shift, achieving a final success rate of  90\%.

% With the checkers pattern the success rate of the zero-shot policy comes down to XX \%. After \iti adaptation, the policy achieves XX \%.


%%%% Figure
\begin{figure}[!t]
    \centering
    \begin{subfigure}[t]{0.34\linewidth}
    \includegraphics[width=\linewidth]{illustrations/gym-fetch.png}
    \end{subfigure}
    \hspace{2em}
    \begin{subfigure}[t]{0.34\linewidth}
    \includegraphics[width=\linewidth]{illustrations/ur5-square-image3.png}
    \end{subfigure}\hfill
    %\vspace{1.6em}
    \caption{Simulated and real reach environment. The goal location is denoted as a red disk that the robot must reach. Using \ac{ILA}, we can transfer a policy trained in simulation (left) onto a real UR-5 robot (right). This adaptation requires no paired data and no rewards on the deployment environment, instead employing \ac{ILA} for unpaired adaptation.}
    \label{fig:sim2real}
\end{figure}


\subsection{Further Discussion}


%\paragraph{Unsupervised Pipeline Ablations} To verify that each component of our unsupervised pipeline contributes to the performance gain during adaptation, we run \iti while setting either the inverse-dynamics or adversarial training losses to $0$. In these experiments, we use a pre-trained DrQ-v2 for the algorithm's base policy, and then run adaptation across all distractions with intensity $0.6$. The results in Table \ref{table:ablation} shows that the adversarial training is critical for the unsupervised pipeline to learn properly. Surprisingly, setting the inverse dynamics loss to zero can actually help performance, suggesting that the encoder has less issues with non-stationary training objectives when it is not also forced to memorize pixel-space dynamics. We note that the inverse dynamics loss was only meant to serve as an auxiliary loss to stabilize training, and that its overall importance in the \iti pipeline is tertiary, as demonstrated by these results.  

% \begin{table}[!ht]
%     \centering
%     % \caption{Impact of adversarial training}
%     \caption{Ablations with variants of \iti, by removing inverse, forward dynamics or adversarial training. DrQ-v2 is used as a pretrained policy. The episode returns are computed from nine domains and five random seeds, and the results correspond to an intensity value of $1.0$.} \label{table:ablation}
%     \begin{tabularx}{1.02\linewidth}{Xcccccc}
%     \toprule
%                  &           &      & +ITI & +ITI & +ITI & +ITI\\
%     Distraction  & Zero-shot & +ITI & w/o inv., fwd. & w/o inv. & w/o fwd. & w/o adv. \\
%     \midrule
% Background & $228 \pm 232$ & $602 \pm 300$ & $615 \pm 289$ & $610 \pm 288$ & $595 \pm 301$ & $176 \pm 221$ \\
% Colors  & $234 \pm 245$ & $536 \pm 320$ & $534 \pm 327$ & $533 \pm 320$ & $515 \pm 331$ & $117 \pm 96\hphantom{0}$ \\
% Camera Pose & $345 \pm 287$ & $417 \pm 284$ & $407 \pm 272$ & $442 \pm 283$ & $429 \pm 274$ & $208 \pm 235$ \\
%     \bottomrule
%     \end{tabularx}
% \end{table}
%
%



\paragraph{Ablation Studies} In order to better understand the contribution of the different objectives to test-time generalization, we perform a series of ablations in which we omit either the dynamics consistency or the adversarial objectives.
% To verify that the adversarial training scheme actually contributes to the performance gain during adaptation, 
%
% This corresponds to an approach that relies purely on the dynamics consistency objective to adapt the latent representation, i.e., the joint objective (Eqn.~\ref{eqn:joint_objective}) becomes $\argmin_F \; \mathcal{J}_\textrm{dyn}$.
%
In these experiments, we use a pretrained DrQ-v2 network for the algorithm's base policy, and then perform adaptation across all distractions with an intensity value of $1.0$. 
The results in Table \ref{table:ablation} show that the adversarial training is critical to adapt the latent representation in the target domain. Performing adaptation using only the dynamics consistency objective, i.e., $\argmin_F$ $\mathcal{J}_\textrm{dyn}$ (Eqn.~\ref{eqn:dynamics_consistency_loss}) results in a significant decrease in performance.
We theorize that the dynamics consistency objective helps to align latent transition manifolds when the latent distributions in source and target domains are reasonably close. 
% to refine the local consistency in the latent spaces when the space in the target domain is close to that of the source domain.
% If the latent spaces significantly differ, 
If the latent distributions significantly differ, however, the input to the pretrained dynamics networks is largely out-of-distribution, and thus the gradients from dynamics consistency loss may negatively affect convergence. % with the right direction to which the latents need to shift.
% only when the latent spaces are already well aligned. 
% and thus it rather harms when the latent spaces largely differ. % Better wording???,  Maybe "shifted", "deviated", "mismatched"? "misaligned" doesn't sound right in this context.

\begin{table}[b!]
    \centering
    \caption{Ablations with variants of \ac{ILA} that remove inverse/forward dynamics, or the adversarial objectives. DrQ-v2 is used as a pretrained policy. We compute episodic returns from nine domains and five random seeds, and the results correspond to an intensity value of $1$.} \label{table:ablation}
    {\small \begin{tabularx}{\linewidth}{Xccccc}
    \toprule
                 &           &      & +ILA & +ILA \\
    Distraction  & Zero-shot & +ILA & w/o dyn. & w/o adv. \\
    \midrule
    Background & $228^{\scriptscriptstyle\pm 232}$ & $602^{\scriptscriptstyle\pm 300}$ & $615^{\scriptscriptstyle\pm 289}$ & $176 ^{\scriptscriptstyle\pm 221}$ \\
    Colors  & $234^{\scriptscriptstyle\pm 245}$ & $536^{\scriptscriptstyle\pm 320}$ & $534^{\scriptscriptstyle\pm 327}$ & $117 ^{\scriptscriptstyle\pm 96}\hphantom{0}$ \\
    Camera Pose & $345^{\scriptscriptstyle\pm 287}$ & $417^{\scriptscriptstyle\pm 284}$ & $407^{\scriptscriptstyle\pm 272}$ & $208^{\scriptscriptstyle\pm 235}$ \\
    \bottomrule
    \end{tabularx}}
\end{table}
%
%
% Why w/o adv. drops performance significantly
% ==> Why dynamics consistency loss is not enough
Compared to the adversarial objective, ablating the dynamics consistency objective
has surprisingly little effect on test-time generalization. 
%$ More detailed ablation results are in Appendix \ref{app:ablations}. 
% Adaptation without dynamics consistency loss surprisingly achieves as good performance as the full model.
It may be that the transition manifold in latent spaces
% local structure of the latents 
are preserved despite the distractions, which then diminishes the net effect of the dynamics consistency objective. 
%For example, one can think of the case where the latents in target domain is shift and affine-transformation of latents in a source domain.
% is shifted and affine-transformed. 
%In such a case, solely matching the latent distributions can effectively match all the latents.
% undo the transformations, resulting in a representation that is consistent with the original
%, without the need to explicitly align local structure. We suspect that this may be the case in the domains that we considered, and thus the effect of dynamics consistency objective gets obfuscated.
%\todoty{Actually I have a very interesting result where the inv and fwd dynamics loss goes down even when we use adversarial objective only. This supports the hypothesis I wrote, and we may put the plot in Appendix. But this makes readers wonder more as to why we didn't stop using dynamics consistency loss in the main results.}
% This indicates that matching latent distributions via the adversarial objective often aligns local consistency in the latent space altogether.

% We theorize that the inverse dynamics head has a tendency to simply memorize dynamics in the training and testing domains without collapsing the commonalities, i.e. it memorizes rather than learns. The adversarial training component ensures that the learning is projected onto a latent space that is agnostic of the underlying MDP.   


%Surprisingly, setting the inverse dynamics loss to zero can actually help performance, suggesting that the encoder has less issues with non-stationary training objectives when it is not also forced to memorize pixel-space dynamics. We note that the inverse dynamics loss was only meant to serve as an auxiliary loss to stabilize training, and that its overall importance in the \iti pipeline is tertiary, as demonstrated by these results.  


%Setting the inverse dynamics loss to $0$ does degrade performance, but its importance is clearly secondary.


%On the other hand, stripping inverse dynamics does not entirely collapse the adaptation.
%Takuma --- Need to add: why it works without inv-dynamics
%\takuma{I'll add the results and its analysis tonight}
%\matt{We might want to consider transposing the tables, with one row for each method and one column or each experiment}

% ^ these numbers are calculated from the separate runs from the main plot (intensity vs return). Also, these use the episode return at the end of adaptation, rather than max return during adaptation (main plot)

% After ICLR submission:
% \subsection{Robotics Manipulation}
\paragraph{Pre-Filling The Replay Buffer}
We implicitly make the assumption that a behavior policy $\bar{\pi}$ is available that can be used to generate trajectory data on both the source and the target domain with similar state visitation, and transition probabilities. To achieve good performance with the adapted policy, such distribution should also cover important states with higher reward. To our surprise, a simple scheme where we pre-fill both the source and target buffer using the random policy works sufficiently well.
% and (2) covers the states relevant to performing a task. Pre-filling both buffers with a random policy was good enough to perform adaptation successfully in our experiments, however, cleverer exploration strategy may be required in some hard-exploration environments.
% In our experiments, we pre-filled both the original latent buffer and the target observation buffer with data collected via random exploration. 
% There is nothing particularly special about this choice, random exploration may be subbed out with any exploration strategy. 
% One interesting strategy is to pre-fill the buffer with an exploration strategy that relies on unsupervised pretraining. Given the recent success of these strategies on improving exploration, it seems likely this could further improve performance. We leave this for future work.

%\todomw{cite APT and APS}.\todomw{I don't remember adding this comment :-)}

%Many approaches have been studied in the line of unsupervised reinforcement learning~\citep{}.\todomw{Update} Recently, exploration strategies framed as unsupervised pretraining have shown to significantly improve performance on a variety of downstream tasks~\citep{}.\todomw{cite APT and APS} Adopting these strategies as the exploration policy for pre-filling\todomw{Be consistent wrt ``pre-filling'' vs ``prefilling''} the buffer may improve the adaptation performance even further. This is left for future work.



%\paragraph{Only fine-tuning the layer norm (tent)}
% \paragraph{Architectures: ViT vs CNN}

==> sections/introduction.tex <==
\section{Introduction}

Reinforcement learning for control has achieved great success in a wide variety of challenging sensory-motor control tasks, including agile drone flight~\cite{Kaufmann2018drone,Kaufmann2020drone,Loquercio2021drone}, deformable object manipulation~\cite{Wu2019deformable}, and quadruped locomotion~\cite{Hwangbo2019agile,Miki2022wild,Lee2020terrain,margonlis2022rapid}. In comparison to their classical model-predictive control counterparts, reinforcement learning-based approach enables the use of more realistic forward dynamics model in the form of a physics simulator, where the controller can be exposed to a larger variety of failure cases that are either unsafe, or otherwise infeasible to experiment with on a physical robot. Improvements in rigid-body simulator technologies~\cite{Todorov2012mujoco,Makoviychuk2021Isaac} also allows reinforcement learning algorithms to by-pass the prohibitively-high sample complexity. A key problem that remains is how to bridge the sim-to-real gap. In particular, how to produce visuomotor control policies that remain robust under a large variety of perceptual conditions, remains an open problem.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{illustrations/motivation/motivation_v6.pdf}%
    % \includegraphics[width=\linewidth]{illustrations/motivation/motivation_v5.pdf}\hfill
    % \includegraphics[width=0.45\linewidth]{illustrations/motivation/iti_v1.pdf}
    \caption{Data augmentation improves the coverage of the training distribution at the expense of learning complexity and performance. 
    %When the sim-to-real gap is large, such method often fail to adequately cover the targeted distribution at deployment. Blue (dashed) distribution indicates the original source. Green (solid) distribution indicates the augmented data. Pink distribution indicates the test distribution the robot experiences at deployment. 
    Insets: (a, c) augmented training data; (b) the original input image from the source domain; %(d) a photo of the setup at deployment; 
    and (d) the input image in the target domain. Data augmentation fails to provide sufficient coverage of the unknown deployment condition, so the learned controller fails to accomplish the task.}\label{fig:out-of-distribution}
\vspace{-1em}
\end{figure}
%
Consider the illustration in Figure~\ref{fig:out-of-distribution}. A common approach to battle domain shift, is to expose the agent during training to a large variety of data with the hope that the training distribution provide coverage over what the agent experiences in the wild. When the simulator is extensible, one can use domain randomization to generate more diverse training data~\cite{Tobin_2017}. Alternatively one can use data augmentation mechanisms to decorate existing data~\cite{yarats2021drqv2,hansen2020deployment}. Both approaches aim to produce visual features that are invariant to perceptual changes orthogonal to the task. Such invariance does not come for free, however. Additional training slows down the wall-clock speed of the training process, whereas the randomization itself requires manual tuning~\cite{Andrychowicz2020dexterous}. The added complexity can negatively affect model and policy performance~\cite{laskin2020reinforcement,hansen2020deployment}. Further more, hidden beneath is the assumption that one needs to know roughly what types of perceptual shift would occur during deployment. Failure can happen when the target domain is not known \textit{a priori} and falls \textit{out-of-distribution}, resulting in a fumbling robot that is unable to self-correct (see Figure~\ref{fig:out-of-distribution}). %Thus, the failure case illustrated in Figure~\ref{fig:out-of-distribution} where the UR5 robot arm is out-of-distribution of the augmented training data is a norm in the wild, rather than an exception.

Different from these prior approaches that produce invariance by memorizing what is irrelevant to the task during training, a more challenging, but also more realistic scenario is one in which the specifics of the deployment is \textbf{not known} before hand. This requires the agent to generalize truly \textit{out-of-distribution} without prior knowledge of the target environment. We further assume that instrumented reward supervision is unavailable, so fine-tuning via REINFORCE is out of the question. This might seems to be an impossible task, but it does implicitly make the assumption that the same \textit{task} the agent was optimized for during training remains well-defined in the target domain. This means that the agent have \textit{some} notion of \textit{what it knows} despite of the sudden appearance of many unknowns that are not required for the task of interest. Without further assumptions or loss of generality, this \textit{out-of-distribution} generalization problem can be formulated as \textit{unsupervised policy adaptation} between two MDPs that share the same latent dynamics and reward structure, but with distinct pixel observations. 
% Similar approaches in supervised learning and computer vision were referred to as unsupervised domain adaptation, train-on-test, and tailoring.



\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{illustrations/latent_projection.pdf}
    % \caption{Distribution shift in observation space causes misalignment in the latent features. ILA adapts projection in order to bring back the latent feature distribution to that of source domain. We formulate this as a distribution-matching objective in Section~\ref{sec:dist_matching}}
    \caption{
    Latent features of the network experience a covariant shift in the target domain. ILA counteracts this domain shift by projecting the features back to the known distribution of latent features on the source domain. We formulate this as a distribution-matching objective in Section~\ref{sec:dist_matching}.
    }\label{fig:out-of-distribution}
\vspace{-1em}
\end{figure}

% This type of unsupervised adaptation in RL has not yet been widely explored, to the best of our knowledge. One of the simplest approaches in this vein is to train a policy with a self-supervised auxiliary task such as inverse dynamics, and rely entirely on it during adaptation \citep{padhansen2020selfp}. Although attractive for its simplicity, this approach often performs poorly in practice, as discussed in Section \ref{sec:experiments}. We also note that this requires the training to be done with a specific auxiliary task, whereas ILA can work with any pretrained policy.
% Another approach is to enforce a Cycle-GAN \citep{zhu2017unpaired} style objective to learn cycle-consistent mappings between domains \citep{zhang2021policy, zhang2021cycle-consistency}. Although this is shown to work well in multiple scenarios, it requires access to states, which are not generally available in the pixel-based control tasks we consider.

% Takuma edited (original is right above)
In this paper, we investigate ways to improve generalization under this challenging scenario. Rather than battling domain shift by baking perceptual invariance explicitly into the network during training, we demonstrate a way to produce feature invariance \textit{at the time of deployment} by taking advantage of the knowledge that the agent has already acquired during training. Our approach, invariance through latent alignment, uses collections of latent features collected during training as examples of what the agent \textit{knows} about the task. On the target domain we then collect new latents that are now shifted from these prior distributions, and cast the unsupervised policy adaptation problem as matching the distribution of latent features on the current, target domain with those that occurs on the source domain during training. This self-supervised learning objective, which we refer to as \textit{latent alignment}, does not require paired image data between the source and the target, and can be applied to any agent without putting specific requirements of how it is trained. To distinguish our approach from prior works that attempt to produce generalization by baking invariances into the policy at training time, we refer to our method as ``\textit{\ila}.''

% Ge original

%The ability for an intelligent agent to generalize can take two different forms: a weaker, and much easier problem formulation looks at the ability for the agent to generalize in-distribution, where one assumes that the agent experiences variation during training that are sufficient to  generalize during deployment. Approaches such as domain transfer, domain randomization and meta learning all fall into this category. Failure can happen when the target domain is not known \textit{a priori} and falls \textit{out-of-distribution}, resulting in a failed agent that is unable to self-correct.

%A more challenging, but also more realistic scenario is one in which the specifics of the deployment is \textbf{not known} before hand. This requires the agent to generalize truly \textit{out-of-distribution} without prior knowledge of the target environment. We further assume that instrumented reward supervision is unavailable, so fine-tuning via REINFORCE is out of the question. This might seems to be an impossible task, but it does implicitly make the assumption that the same \textit{task} the agent was optimized for in the factory\todomw{factory?} remains well-defined in the target domain, which means that the agent does have \textit{some} notion of the underlying Markov decision process. Without further assumptions or loss of generality, we define this \textit{out-of-distribution} generalization problem to be an \textit{unsupervised policy adaptation} between two MDPs that share a similar latent dynamics and reward structure, but with distinct observations.

%In this paper, we investigate ways to solve generalization under this challenging scenario. Instead of producing policy invariance by explicitly pre-programming this property in, we produce invariance using what the agent already knows, through probabilistic inference. Much of our focus is on producing agents that can function effectively in environments that exhibit different  lighting, object texture, or camera poses in a three-dimensional robotics domain. We also demonstrate the ability for our method to generalize across forward dynamics that are different, as long as the some resemblance remains in-between.\todomw{``some resemblance remainds in-between''?}

%Hence to distinguish our approach from prior works that attempt to produce generalization by baking invariances into the policy at training time, we refer to our method as ``\textit{(policy) Invarivance Through Inference}''.

==> sections/invariance_through_inference.tex <==
\section{\ila}
%
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{illustrations/main_fig/ILA_v2.pdf}
    \caption{Training and adaptation phases of \lcila. The encoder $F$ takes an observation of target domain, and learns to fool the discriminator, while the discriminator $D$ predicts whether the input is an encoded target observation or a latent sample from source buffer. This adversarial training encourages the distribution of encoder outputs to be similar to the latent embedding sampled from the source buffer. $C_\textrm{dyn}$ is the pretrained forward and inverse dynamics networks used only to guide the encoder during adaptation.}
    \label{fig:main-fig}

\end{figure*}
%
%

% Following the previous discussion, consider a setting with source and target domains $\mathcal{M}_\textrm{src}$ and $\mathcal{M}_\textrm{tgt}$ that share similar state dynamics and reward structure, however the observation spaces exhibit significant distributional shift. Consequently, an agent trained in the source domain will generally perform poorly in the target domain due to distributional shift in the latent encoding on which the policy is conditioned.


% Following the previous discussion, consider a setting with source and target domain $\mathcal{M}_\textrm{src}$ and $\mathcal{M}_\textrm{tgt}$. An agent trained in the source domain will generally perform poorly in the target domain due to distributional shift in the latent representation on which the policy is conditioned.


% Our algorithm, \iti,  learns a feature extractor that maps semantically similar observations to close latent vectors, learning to ignore irrelevant distractions in the observation space, without access to target rewards. We achieve this through two primary objectives: \textit{distribution matching loss} that encourages the latent distributions to match (i.e., aligning global latent structure); and \textit{dynamics consistency losses} to  encourage to match the latent dynamics (i.e., aligning local latent structure).


%When we deploy the pre-trained agent in the unseen target domain, due to the distributional shift in the observation space, the distribution over the encoded latent $z$ largely differs from what the pre-trained policy $\pi(a|z)$ has seen during training.
%We believe this is the main cause of the performance drop.\todomw{We just said this a few lines above}
%To fix this via adaptation, we have two objectives: \textit{distribution matching loss} to encourage the latent distributions to match (aligning global latent structure); and \textit{dynamics consistency losses} to  encourage to match the latent dynamics (aligning local latent structure).

\subsection{Distribution Matching}\label{sec:dist_matching}

For simplicity, we consider trajectories of observation and actions collected via a random policy in both the source and the target domain.
%
\begin{subequations}
    \begin{align}
        \mathcal{B}_\src = \left(\ldots, o_t^{\src}, a_t^{\src},  o_{t+1}^{\src}, \ldots \right) &\sim  P_{\bar{\pi}}(\mathcal{M}_{\text{src}})\label{eqn:src_buffer},\\
        \mathcal{B}_\tgt = \left(\ldots, o_t^{\tgt}, a_t^{\tgt}, o_{t+1}^{\tgt}, \ldots \right) &\sim  P_{\bar{\pi}}(\mathcal{M}_{\text{tgt}}),\label{eqn:tgt_buffer}
    \end{align}
\end{subequations}
As illustrated in Figure~\ref{fig:main-fig}, we save latent features from the source domain in a buffer. $P_{\bar{\pi}}(\mathcal{M})$ are transitions conditioned on the random policy \(\bar\pi\). % $\mathcal{M}$.
% It should be reminded that we do not have access to reward in target domain.
Given an observation $o_t$, an encoder $F$ produces a latent representation $z_t$. We denote those given on the source domain \(o_t^\text{src}\) and the target domain \(o_t^\text{tgt}\) as%
\begin{subequations}
    \begin{align}
        z_t^{\src} &= F_{\theta_0}(o_t^{\src}),\\
        z_t^{\tgt} &= F_\theta(o_t^{\tgt}),
    \end{align}
\end{subequations}%\todomw{I added $\theta$ to $F$ to make the parameterization explicit. If we keep it, we should make sure that the notation is consistent, i.e., we include $\theta$ elsewhere and change the optimization to be over $\theta$.}
%
where $\theta_0$ indicates the weights of the network are are frozen during adaptation.
We seek to match the distribution of $z_t^{\tgt}$ with $z_t^{\src}$ by adapting the weights of the encoder $F$, without access to paired-images. 
% want to match the distributions of respective latent distributions: % $P_{F}(z|o^{\text{src}})$ and  $P_{F}(z|o^{\text{tgt}})$.
We introduce an adversarial objective (see Figure~\ref{fig:main-fig}), where a discriminator $D$ tries to distinguish between embeddings from the source domain $z^{\src}_t$ and those from the target domain $z^{\tgt}_t$. We update the parameters of the encoder such that latent embeddings on the target domain are indistinguishable. This results in matching latent distribution over $z_t^{\src}$ and $z_t^{\tgt}$. Following the Wasserstein GAN \citep{arjovsky2017wasserstein} formulation, we express our distribution matching loss as
%
%
\begin{equation}
    \begin{split}
    \mathcal{J}_\textrm{adv} = \mathbb{E}_{P_{\bar{\pi}}(\mathcal{M}_\src)} \left[ &D\left(F_{\theta_0} (o^{\text{src}}_t)\right) \right] \\
    %
    &+ \mathbb{E}_{P_{\bar{\pi}}(\mathcal{M}_\tgt) }\left[1 - D\left(F_\theta(o_t^{\text{tgt}})\right) \right].
    \end{split}
% \mathcal J_\text{d} = \argmin_D \bigg[  (1 - \log P(z)) + \log P(\tilde z)
\label{eqn:adversarial_loss}
\end{equation}
%
%
% where $\bar{F}$ indicates that the weights of the network are frozen. 
The encoder tries to minimize this objective while the discriminator acts as an adversary and seeks to maximize it, resulting in a GAN-like minimax game.

% In practice, before adaptation, we apply pre-trained $F$ to observations and store random latent transitions (z_t, a_t, z_{t+1}) to \textit{source buffer}. During adaptation, we sample from 



\subsection{Dynamics Consistency}
% Adversarial training can, in theory, learn mappings G and F that produce outputs identically distributed as target domains Y and X respectively (strictly speaking, this re- quires G and F to be stochastic functions) [15]. However, with large enough capacity, a network can map the same set of input images to any random permutation of images in the target domain, where any of the learned mappings can induce an output distribution that matches the target dis- tribution. Thus, adversarial losses alone cannot guarantee that the learned function can map an individual input xi to a desired output yi.
% ^ This is a quote from Cycle GAN!

Theoretically, the use of adversarial training can result in an encoder that maps source and target domain observations to latent embeddings that have identical distributions. However, it is possible for a sufficiently expressive encoder to map the same target observations to a random perturbation of observations in the source domain while still matching the distributions~\citep{zhu2017unpaired}. To mitigate this, we take advantage of the shared underlying dynamics as a feature-rich and informative source of mutual information between the two domains. %The \textit{dynamics consistency loss} helps to avoid such solutions.

% Specifically, let $C_{\text{fwd}}(z_t, a_t)$ denote a forward dynamics network that predicts the next latent representation $z_{t+1}$ given the current latent embedding $z_t$ and action $a_t$. Similarly, let $C_{\text{inv}}(z_t, z_{t+1})$ be the inverse dynamics network that predicts the action $a_t$ associated with the transition from $z_t$ to $z_{t+1}$. 
 Specifically, let $C_{\text{inv}}(z_t, z_{t+1}; \psi_\textrm{inv})$ be the inverse dynamics network that predicts the action $a_t$ associated with the transition from $z_t$ to $z_{t+1}$, and $C_\textrm{fwd}(z_t, a_t; \psi_\textrm{fwd})$ be the forward dynamics network that predicts the next latent $z_{t+1}$from $z_t$ and $a_t$.
We then define the \emph{dynamics consistency loss} as the error in the 
forward and inverse dynamics predictions

%
%
\begin{equation} \label{eqn:dynamics_loss}
    \begin{split}
        \mathcal{L}_\textrm{dyn}(z_t, z_{t+1}, a_t; &\psi_\textrm{fwd}, \psi_\textrm{inv}) = \lVert C_{\text{fwd}}(z_t, a_t; \psi_\textrm{fwd}) - z_{t+1} \rVert_2^2\\%
        &+ \lambda \lVert C_{\text{inv}}(z_t, z_{t+1}; \psi_\textrm{inv}) - a_t \rVert_2^2,
    \end{split}
\end{equation}
%
%
where $\lambda$ is a hyperparameter that corrects for scaling differences. % between the forward and inverse dynamics components of the loss.

Most importantly, we pretrain the 
forward and inverse dynamics networks on
transitions sampled from the source domain 
$\mathcal{B}_\src \sim P_{\bar{\pi}}(\mathcal{M}_\src)$
% $\mathcal{M}_\src$
(Eqn.~\ref{eqn:src_buffer}) with observations encoded with $F_{\theta_0}$.
% We denote this $\mathcal{B}^*_\src \sim P_{\bar{\pi}}(\mathcal{M}_\src; F_{\theta_0})$
\begin{align}
\psi_\textrm{fwd}^*, \psi_\textrm{inv}^* = \underset{\psi_\textrm{fwd}, \psi_\textrm{inv}}{\textrm{arg min}} \; 
&\mathbb{E}_{P_{\bar{\pi}}(\mathcal{M}_{\src}; F_{\theta_0})} \big[ \nonumber \\
&\mathcal{L}_\textrm{dyn}(z^{\src}_t, z^{\src}_{t+1}, a^{\src}_t; \psi_\textrm{fwd}, \psi_\textrm{inv}) \big] 
    \label{eqn:dynamics-pretrain} 
\end{align}
%
%
% %
% %
% \begin{equation}
%     \begin{aligned}
%         \psi_\textrm{fwd}^*, \psi_\textrm{inv}^* = \underset{\psi_\textrm{fwd}, \psi_\textrm{inv}}{\textrm{arg min}} \; 
%         &\mathbb{E}_{P_{\bar{\pi}}(\mathcal{M}_{\src}; \bar{F})} \left[ \\
%         &\mathcal{L}_\textrm{dyn}(z^{\src}_t, z^{\src}_{t+1}, a^{\src}_t; \psi_\textrm{fwd}, \psi_\textrm{inv}) \right],
%         \label{eqn:dynamics-pretrain} 
%     \end{aligned}
% \end{equation}
% %

%After training these on transitions from $P_{\bar{\pi}}(\mathcal{M}_\src)$, we can safely say that these models implicitly encode the structure of latent transition dynamics. 
% where we use $\mathcal{L}_\textrm{dyn}^\textrm{src} = \mathcal{L}_\textrm{dyn}(z^{\src}_t, z^{\src}_{t+1}, a^{\src}_t; \psi_\textrm{fwd}, \psi_\textrm{inv})$ for lack of space and $P_{\bar{\pi}}(\mathcal{M}; \bar{F})$ is the distribution over latent trajectories.
Under the assumption that the underlying dynamics are shared by the domains, we then utilize these learned 
dynamics models to further encourage the latent embeddings for the target domain to align with those of the source domain. Specifically, during adaptation, we freeze the weights of the 
forward and inverse dynamics networks, and minimize the following dynamics consistency loss with respect to encoder $F$ using transitions sampled from the target domain $\mathcal{B}_\tgt \sim P_{\bar{\pi}}(\mathcal{M}_\tgt)$ (Eqn.~\ref{eqn:tgt_buffer}) 
%
%
\begin{equation}
    \mathcal{J}_\textrm{dyn} =  \mathbb{E}_{P_{\bar{\pi}}(\mathcal{M}_\tgt; F_\theta)} \left[ \mathcal{L}_\textrm{dyn}(z^{\tgt}_t, z^{\tgt}_{t+1}, a^{\tgt}_t; \psi^*_\textrm{fwd}, \psi^{*}_\textrm{inv})\right].
    \label{eqn:dynamics_consistency_loss}
\end{equation}
%
%

%Formally, we consider the objective
%
%
%\begin{equation}
%    F^* = \underset{F}{\textrm{arg min}} \;  \mathbb{E}_{P_{\bar{\pi}}(\mathcal{M}_{\tgt}; F)}
%    \left[ \mathcal{J}(z^{\tgt}_t, z^{\tgt}_{t+1}, a^{\tgt}_t) \right],
%    \label{eq:dynamics-consistency}
%\end{equation}
%
%
%where, with abuse of notation, $P_{\bar{\pi}} (\mathcal{M}; F)$ denotes the distribution over latent transitions produced with sampling from $P_{\bar{\pi}}(\mathcal{M})$ followed by applying $F$ to the observations.
% The difference from Equation \ref{eq:dynamics-pretrain} is marked in red for the purpose of visual aide.
%This objective guides the feature extractor to meet the same latent transitions as they were in source domain.

\subsection{The Full Learning Objective}

% \takuma{I need advice on how I can simplify this algorithm box. Especially the parts calculating gradient and updating weights can be somehow merged.}
\begin{algorithm}[t]

% \todoty{I want to know how to simplify the algorithm box further}
\caption{\ila}\label{alg:cap}
\begin{algorithmic}
\small
\Require Pretrained encoder $F_{\theta_0}$, discriminator $D_\phi$, buffers $\mathcal{B^{*}_\src}$ and $\mathcal{B_\tgt}$, inverse dynamics network parameterized with $\psi_\textrm{inv}$
% \Ensure $y = x^n$
% \State $N \gets n$
\For{i=1:N} \Comment{Pre-fill buffers}
\State \text{Sample} $z_t, a_t, z_{t+1} \sim P_{\bar{\pi}}(\mathcal{M}_\src ; F_{\theta_0})$
\State \text{Sample} $o_t, a_t, o_{t+1} \sim P_{\bar{\pi}}(\mathcal{M}_\tgt)$
\State $\mathcal{B}^{*}_\src \gets \mathcal{B}^{*}_\src \cup (z_t, a_t, z_{t+1})$
\State $\mathcal{B}_\tgt \gets \mathcal{B}_\tgt \cup (o_t, a_t, o_{t+1})$
\EndFor

\For{$i=1:T_\text{dynamics}$}  \Comment{Pretrain dynamics networks}
\State \text{Sample} $z_t, a_t, z_{t+1} \sim \mathcal{B}^*_\src$
\State $g_\text{fwd}, g_\text{inv} \gets \nabla_{\psi_{\text{inv}}}\mathcal{L}_\textrm{dyn}(z_t, z_{t+1}, a_t; \psi_\textrm{fwd}, \psi_\textrm{inv})$
% \State $g_\text{fwd} \gets \nabla_{\phi_{\text{fwd}}}\mathcal{J}(z_t, z_{t+1}, a_t)$
\State $\psi_\text{fwd}, \psi_\text{inv} \gets \text{Optimizer}(\psi_{\text{fwd}}, \psi_{\text{inv}}, g_{\text{fwd}}, g_{\text{inv}})$
% \State $\phi_\text{fwd} \gets \text{Optimizer}(\phi_{\text{fwd}}, g_{\text{fwd}})$
\EndFor

\For{$i=1:T_\text{adapt}$}  \Comment{Adaptation main loop}
\State \text{Sample} $z^{\src}_t, a^\src_t, z^\src_{t+1} \sim \mathcal{B}^*_\src$
\State \text{Sample} $o^\tgt_t, a^\tgt_t, o^\tgt_{t+1} \sim \mathcal{B}_\tgt$
\State $g_D \gets \nabla_{\phi} \big[ D_\phi(z_t^{\src}) + (1 - D_\phi(F_\theta(o_t^{\tgt}))) \big]$ \Comment{Distr. matching}
\State $g_{F_1} \gets \nabla_{\theta} \big[ D_\phi(z_t^{\src}) + (1 - D_\phi(F_\theta(o_t^{\tgt}))) \big]$
\State $g_{F_2} \gets \nabla_{\theta} \mathcal{L}_\textrm{dyn}(F_\theta(o_t^{\tgt}), F_\theta(o_{t+1}^{\tgt}), a_t; \psi_\textrm{fwd}^*, \psi_\textrm{inv}^*)$  \Comment{Dynamics consistency}
\State $\phi \gets \text{Optimizer}(\phi, g_D)$
\State $\theta \gets \text{Optimizer}(\theta, g_{F_1}, g_{F_2})$
%
\EndFor
%
\end{algorithmic}
\label{alg:adaptation}
\end{algorithm}

% \begin{figure}{\textwidth}
% \vspace{-2em}
%     \includegraphics[width=0.8\linewidth]{illustrations/distractor_scale/distractor_scale.pdf}
%     \caption{Samples from the modified \textit{distracting control suite}. Top row: color, middle row: background distractions, bottom row: camera pose.}
%     \label{fig:distractions}
% \end{figure}%


\begin{figure*}[t]
    \begin{minipage}{0.34\textwidth}
    \includegraphics[width=\linewidth]{illustrations/distractor_scale/distractor_scale.pdf}
    \caption{Samples from the modified \textit{distracting control suite}. Top row: color variations, middle row: background distractions, bottom row: camera pose variations.}
    \label{fig:distractions}
    \end{minipage}\hfill%
    \begin{minipage}{0.63\textwidth}
  \begin{subfigure}[t]{0.3\linewidth}
    \centering
    \includegraphics[height=80px]{results/intensities-20220505/color.pdf}
    \caption{Color}
    \label{fig:intensity-colors}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.3\linewidth}
    \centering
    \includegraphics[height=80px]{results/intensities-20220505/background.pdf}
    \caption{Background}
    \label{fig:intensity-background}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.3\linewidth}
    \centering
    \includegraphics[height=80px]{results/intensities-20220505/camera-with-legend.pdf}
    \caption{Camera Pose}
    \label{fig:intensity-camera}
  \end{subfigure}
    \vspace{0.5em}
    \caption{The gain of applying \ac{ILA} to target domains with various distraction intensities. Dashed lines denote the performance of the baseline agent in the target environment (i.e., zero-shot transfer), while solid lines represent the performance gains of the agents with ILA.}% \takuma{Issues: (1) matplotlibrc seems not be active, thus string are tiny; (2) Somehow the label on y-axis (episode reward) is gone only on pdf, but not on png; (3) legend never shows up. Need to ask Ge for help.} \matt{We should use PDF whenever we can (assuming the graphic is vector-based)}}
    \label{fig:intensity-vs-reward}
  \end{minipage}
\end{figure*}
%
%

We adapt our encoder by minimizing a loss that combines both the adversarial loss $\mathcal{J}_\textrm{adv}$ (Eqn.~\ref{eqn:adversarial_loss}) and the dynamics consistency loss $\mathcal{J}_\textrm{dyn}$ (Eqn.~\ref{eqn:dynamics_consistency_loss}). Specifically, we solve for the parameters of the encoder through the following minimax objective
% \todomw{Are they weighted equally or do we need a $\lambda$}
%
%
\begin{equation}
    \argmin_\theta \argmax_\phi \left[  \mathcal{J}_\textrm{adv} + \lambda^\prime \mathcal{J}_\textrm{dyn} \right],
    \label{eqn:joint_objective}
\end{equation}
%
%
where $\lambda^\prime$ is a hyperparameter that balances the loss terms. This adaptation objective is effectively maximizing the mutual information between the prototypical representation kept from during training, and the adapted representations of the new observations. 
Algorithm \ref{alg:adaptation} summarizes the whole procedures to sample trajectory, pretrain dynamics networks and adapt encoder via the objective.


In summary, in contrast to those methods that produce invariance by exposing the network to various perceptual changes, 
our adaptation scheme produces domain-invariance by aligning their latent representations. 
% For this reason we refer to the derived method as \ila.



% \subsection{Inference}
% \todoty{Tentative title}
% \include{graphical_model}
% \todoty{This is a version very similar to Adversarial Learned Inference paper. This is hand wavy and effectively says nothing.}
% To discuss the interpretation of our adaptation objective, we first define the following probabilities:
% \begin{itemize}
%     \item Observation distributions in source domain: $p^\text{src}(o_t)$
%     \item Observation distributions in target domain: $p^\text{tgt}(o_t)$
%     \item Latent distribution with the pretrained encoder: $p(z_t | o_t)$
%     \item Latent distribution with the adapting encoder: $q_\theta(z_t | o_t)$
% \end{itemize}
% It is noted that observations are sampled by running a random policy.

% Using the notation above, the adversarial objective Eqn. (\ref{eqn:adversarial_loss}) can be expressed as
% \begin{eqnarray}
%     \mathbb{E}_{p^\text{src}(z_t)}[D_\phi(z_t)] + \mathbb{E}_{q^\text{tgt}_\theta(z_t)}[1 - D_\phi(z_t)] \\
%     = \int p(z_t|o_t)p^\text{src}(o_t)D_\phi(z_t) do_t  \\
%     + \int q_\theta(z_t|o_t) p^\text{tgt}(o_t)\{1 - D_\phi(z_t)\} do_t
% \end{eqnarray}
% Our goal here is to obtain the inference probability $q_\theta(z_t|o_t)$ which is characterized by its parameter $\theta$.
% Min-max optimization on this adversarial objective is known to be equivalent to minimizing XX divergence between the distributions over $z_t$. Thus our objective is equivalent to

% \begin{equation}
%     \min_\theta \text{Div}[p(z_t) \| q\theta(z_t)],
% \end{equation}
% where
% \begin{eqnarray*}
% p(z_t) = \int p(z_t|o_t) p^\text{src}(o_t) do_t \\
% q_\theta(z_t) = \int q_\theta(z_t|o_t) p^\text{tgt}(o_t) do_t.
% \end{eqnarray*}
% % Our goal is to minimize the following divergence with respect to $\theta$
% % \begin{eqnarray}
% %     \text{Div}[p^\text{src}(z_t) \| q^\text{tgt}_\theta(z_t)] \\
% %     = \text{Div} \Big[\int p(z_t|o_t)p^\text{src}(o_t) do_t \Big|\Big| \int q_\theta(z_t|o_t) p^\text{tgt}(o_t) do_t \Big]
% % \end{eqnarray}
% -------------------------------------

% \todoty{This is more accurate description of what we do.}


% We jointly optimize these two objectives: \textit{distribution matching loss} and \textit{dynamics consistency loss} during adaptation. We can see this adaptation strategy as aligning the latent spaces. Given an agent pretrained in source domain, 


%\stadie{Done editing. Need serious feedback. Do sections 3.2 and 3.3 make sense to include? Should we just try harder to incorporate information from 3.2 into 3.1? That seems most obvious to me. I need to step back for a minute before I can evaluate this again. @Ge, Takuma, Matt. Please feel free to make changes and improvements.}

%The key insight of this model is that we can leverage XXX to learn representations that are quick to adapt to new environments????\todomw{Update}
% \subsection{A loss function for \iti}
% Following the previous section, assume we are in a setting with two MDPs, $\mathcal{M}_\textrm{train}$ and $\mathcal{M}_\textrm{test}$. We assume these MDPs share similar states, dynamics, and reward structures. However, the observation spaces incur a significant distributional shift. Nevertheless, since the underlying state and dynamics that are relevant to the task are similar, there exists some encoding $z = G_\theta(o, a)$ s.t.
%that preserves some form of continuity between states
%
%
% \begin{align*}
%     \| s_\textrm{train} - s_\textrm{test} \| \leq \delta \to \| G_\theta(o_\textrm{train}, a_\textrm{train}) - G_\theta (o_\textrm{test}, a_\textrm{test}) \| \leq \epsilon
% \end{align*}
%
%
% In other words, we want to learn a latent encoder that maps semantically similar observations to close latent vectors, learning to ignore irrelevant distractions in the observation space. In many real world deployment scenarios, test-time rewards $R_\textrm{test}$ are unavailable. Thus, we have hope to train this encoder without access to test-time rewards. Given this constraint, we note that the shared underlying dynamics are the most feature-rich and informative source of mutual information between the two environments. We would therefore like our encoded latents to minimize an inverse dynamics model loss
%
%
% \begin{equation}
% \mathcal J_\text{inv} = \mathbb{E}_{\substack{o_{t+1} \sim \pi(o_t, a_t) \\ z_t = G_\theta(o_t) \\ z_{t+1} = G_\theta(o_{t+1})}} \bigg[ \lVert P_\phi(z_t, z_{t+1}) - a_t \rVert^2 \bigg]
% % \mathcal J_\text{Inv M} = \argmin_D \bigg[ \log P(z) + (1 - \log P(\tilde z))  \bigg]
% \end{equation}


% However, simply training this model with data from both MDPs will not ensure that observations with similar ground-truth states are actually aligned. Instead, the encoder might simply learn to handle each MDP independently. Critically, we do not assume access to paired trajectories, which can be difficult to achieve in practice. If we had access to such paired data, we could simply train an encoder that minimizes the distance to both paired observations. At minimum, we would like to ensure that the latent distributions over observation embeddings for both MDPs are similar, since that would hopefully force the encoder to filter out superfluous distractions that separate the two MDPs. Towards this goal, we define two objectives. First, a distribution matching objective encourages the latent distribution induced by both MDPs to match.
%
%\matt{Where do we use Equation 3?}
% \begin{equation}
% \mathcal J_\text{d} = \argmin_D \bigg[ \log P(z) + (1 - \log P(\tilde z))  \bigg]
% \end{equation}

%\todomw{It's not clear to me what we are optimizing over, i.e., where is $D$ on the RHS? $P \rightarrow D$?}

% Second, we employ a GAN-style loss to help ensure that the latent code is not using distracting information that would help distinguish the train and test MDPs
%
%
% \begin{equation}
% \mathcal J_D =  \mathbb{E}_{o_t \sim D_\textrm{non-distr}}\big[ \log D(\bar{G}_\theta(o_t)) \big] + \mathbb{E}_{o_t \sim D_\text{distr}}\big[ \log (1 - D(G_\theta(o_t))) \big] \bigg],
% % \mathcal J_\text{d} = \argmin_D \bigg[  (1 - \log P(z)) + \log P(\tilde z)
% \end{equation}
%
% where $\bar{G}$ denotes the encoder whose weights are frozen after training. The final objective can now be written as 
%
%
% \begin{equation} \label{eq:loss}
%     \argmin_{G_\theta} \; \argmax_{D} \bigg[ \mathcal{J}_{D} + \mathcal{J}_\text{inv} \bigg]
% \end{equation}
%
%

% Takuma --- I guess I should add something like this to validate the naming of inv-thru-inf
%                     but with clearer and simpler language.
% This adaptation objective is effectively maximizing the mutual information between the prototypical representation retained during training, and the adapted representations of the new observations. In summary, in contrast to those methods that produce invariance through memorization, our adaptation objective produces invariance by making statistical inference in the latent space. For this reason we refer to the derived method as \iti. 

%\todomw{BCS -- @Ge. We need to address the algorithm's name somewhere. Maybe not here. But somewhere. I'm leaving this stub as a reminder for you to address the situation.}\todomw{We could informally argue that the manner in which we learn the encoder is analogous to inference over the the relevant aspects of the latent state $s_t$}

%Second, we define a GAN-style objective. 

%As we need a structure that can guide the encoder to produce a meaningful embedding for each observation, we adopted inverse dynamics prediction as its auxiliary task

% \GY{Adapted Version of Takuma's Note}

% We assume that the observations in domain A and domain B sampled from two distributions
% \[
% \begin{aligned}
% o_a^t &\sim P(A)\\
% o_b^t &\sim P(B)
% \end{aligned}
% \]

% The objective we maximize is 
% \[
% \begin{aligned}
% \argmax_\phi \mathcal L\\
% \argmin_D \mathcal L_D\\
% \end{aligned}
% \]

% \todoinmw{Takuma, note that $\mathcal{B}_\src$ in the Algorithm contains embeddings $z$, but Eqn.~1 has it containint observations $o$.}
% \todoty{After rewriting the method section, I figured what our method does is quite clear without a dedicated "Algorithm Overview" section. Algorithm box helps to clarify things, too.}
% \subsection{Algorithm Overview}

%\stadie{This whole subsection seems redundant? Maybe we should just try to incorporate some of this text into the previous subsection? Thoughts appreciated. I need some distance from the writing before I can decide.}

% We assume that we have an agent  that is pretrained in source domain, and that contains encoder $F: O \mapsto Z$ and policy $\pi: Z \mapsto A$. 
% Given the pre-trained agent, there are two preparation steps before running adaptation: pre-filling buffers and pretraining dynamics networks.
% First, we deploy random exploration policy on both source and target domain to collect transitions. The observation transitions in source domain $(o_t, a_t, o_{t+1})$ is encoded with $F$ and the retained latent transitions $(z_t, a_t, z_{t+1})$ are stored in source buffer $\mathcal{B}^{*}_\src$. 
% After storing $N$ transitions in the buffer, we pretrain dynamics networks $C_\textrm{fwd}$ and $C_\textrm{inv}$ using samples from it. This concludes the preparation steps.


% Constructing a pipeline to optimize Eqn. \ref{eqn:joint_loss} is fairly straightforward. The architecture is fully represented in Figure~\ref{fig:main-fig}. The algorithm starts by collecting transitions in the source domain and storing the corresponding latents into a source buffer $\mathcal{B}^{*}_\src$. These initial samples are collected under an exploratory policy. In practice, we find random exploration is sufficient for many robotics environments. 

% Once the buffer becomes full (1 million transitions in our experiments), we can draw samples from it to pretrain the dynamics networks.  The networks implicitly model the latent dynamics. With these in hand, we can start adapting the encoder.
% towards the target domain. 
% Since we want to ensure the observation embeddings for the source and target domain follow a similar distribution, we use the optimization framework from adversarial training to constrain the encoder appropriately. Our encoder $F$ is encouraged to produce similar embeddings on both train and test environment observations. The discriminator $D$ learns to classify whether a given input comes from source environment buffer or target environment. 

% Finally, we need a structure that can help guide the encoder to produce a meaningful embedding for each observation. To wit, we add an inverse dynamics head onto our architecture as a type of auxiliary task, under the assumption that train and test time environments share a high degree of overlap in their environmental dynamics.  This head is pre-trained with transitions sampled from the source buffer, and has its weights fixed during adaptation.

%Our adversarial architecture should encourage the encoder to align the shape of distribution with the one from source environment, however, it still does not guarantee that a pair of observations that share the same true state will be mapped to similar embeddings. As we need a structure that can guide the encoder to produce a meaningful embedding for each observation, we adopted inverse dynamics prediction as its auxiliary task. This adds a new head that takes two consecutive embeddings $z_t$, $z_{t+1}$ and predicts the corresponding action $a_t$.
%We pre-trained this head with transitions sampled from the source buffer, and fixed the weights during adaptation.



% ALGORITHM BOX HERE
%\stadie{Ge, I don't think this algorithm box is needed in this draft? It's best in the appendix anyways?}
%\begin{algorithm}
%\caption{Fitted Q Iteration~\citep{}}\label{alg:adaptation_procedure}
%\begin{algorithmic}[1]
%\State Initialize $Q_\theta$, buffer $\mathcal D$ 
%\While{not converged}
%    \State sample $s_t, a_t, s_{t+1}, r_t$ from $\mathcal D$
%    \State compute target $\mathcal B^* Q = r_t + \gamma %\max_{a^*}Q(s', a^*)$  \label{fqi:target}  \Comment{1-step return}
%    \State minimize TD Loss $\mathcal L_\text{TD} = Q(s, a) - %\mathcal B^* Q$   \label{fqi:update}
%    % \State $Q(s, a) \leftarrow r_t + \gamma \max_{a^*}Q(s', a^*)$
%\EndWhile
%\end{algorithmic}
%\end{algorithm}


%To achieve this, we use Generative Adversarial Networks (GANs) \citep{}. In our setup, encoder corresponds to the generator in GANs, and it is encouraged to produce similar embeddings as to the ones sampled from source environment buffer. Whereas the discriminator learns to classify whether the input comes from source environment buffer or target environment. 

%our main concern during adaptation is to match the distribution of embeddings for source environemnt and target environment

%Once the buffer is fulfilled, we pre-train our inverse dynamics networks with its samples. It is trained to predict an action from two consecutive embeddings

%In practise, we store the latent embedding $z_t = G(o_t)$ during training on the clean environment, and sample $z_t$ from the buffer during adaptation, and feed to the first term.

%Our method consists of three primary stages:\todomw{We can probably be more concise here since we detail the stages below} first, it collects transitions in the \textit{source environment} and stores the encoded observations in a buffer; second, it uses samples from this buffer to pretrain an inverse dynamics networks; and in the third stage, the method adapts the encoder on the \textit{target environment}.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{illustrations/method-pret-phase.v4.png}
%     \caption{Preprocessing for \iti. The first stage pre-fills the source buffer with observation embeddings. The second stage then pre-trains the inverse dynamics head using samples from the buffer.}
%     \label{fig:method-prep}
% \end{figure}


%First, we deploy a random policy in the source environment to collect trajectories. In this step, we store the \textit{embeddings} rather than raw image observations. Following \citet{seer}, we augment the image observation in four ways and stored all embeddings to take advantage of augmentations. Storing embeddings in stead of image observations can reduce the amount of data significantly.  % Takuma --- Hmmm maybe it's a bit too redundant?
%Once the buffer is fulfilled, we pre-train our inverse dynamics networks with its samples. It is trained to predict an action from two consecutive embeddings, and we use it during adaptation stage.

% Takuma --- Our method is rather based on conditional GANs 
%Second, we adapt encoder to the target environment. As described in the previous section, our main concern during adaptation is to match the distribution of embeddings for source environemnt and target environment. To achieve this, we use Generative Adversarial Networks (GANs) \citep{}. In our setup, encoder corresponds to the generator in GANs, and it is encouraged to produce similar embeddings as to the ones sampled from source environment buffer. Whereas the discriminator learns to classify whether the input comes from source environment buffer or target environment. 
% Talk about Inverse dynamics
% Takuma --- It sounds a bit verbose.


==> sections/problem_formulation.tex <==
\section{Problem Formulation}
\label{sec:problem}

%\stadie{Updated rough draft. It's somewhat better but it still needs a lot of discussion and iteration. Ready for feedback and discussion (@Takuma, @Ge) -- Oct 4 at 14:10}

%\stadie{Renamed this section Problem Formulation}

% 1. MDP formulation
% 2. Problem formulation: out-of-distribution generalization
% 

%\stadie{I think the best problem formulation section for inspiration is probably DrQ. The problem there is really clear and well presented. My main issue with the current draft is that I wish it was a bit more mathematical with some centered equations. I think that would give it more punch.}

The standard infinite horizon Markov decision process (MDP)~\citep{Puterman2014mdp} is parameterized via the tuple \(\mathcal{M} = \langle S, O, A, R, P, \gamma\rangle\), where \(S\), $O$, and \(A\) are respectively the state, observation, and action spaces, \(P:S\times A\mapsto S\) is the transition function, \(R: S \times A\mapsto \mathbb R\) is the scalar reward, and \(\gamma\) is the discount factor. Recall that the state space $S$ usually represents ground-truth information about the agent's environment, which we assume the agent can not directly access. Instead, the agent receives a stream of observations $o \in O$ that convey information about the environment. In this paper, we assume a fully-observable setting where a single observation carries enough information to decide an appropriate action. The goal of reinforcement learning is to solve for the policy $\pi: O \times A \mapsto [0, 1]$ that maximizes the expected discounted return \(\mathcal J = \mathbb{E}\left[ \sum_\infty \gamma^t R(s_t, a_t)\right]\) over infinite horizon, represented as the \(Q^\pi(o, a)\) function. In this paper, we assume that the policy $\pi$ consists of an encoder $F: O \mapsto Z$, where $Z$ is a compact latent space, and a policy $\pi_z:Z \times A \mapsto [0,1]$.

%\stadie{This might be wrong (do we observe rewards at test time?), but we can fix it if that's the case. It doesn't really ruin this section or anything.}
%\takuma{This is correct :) We don't observe reward during adaptation.}

\input{graphical_model}
%\todoinmw{I have a slight preference for the previous version of the paragraph below.}
We consider a setting wherein there are two distinct domains, a source domain $\mathcal{M}_\textrm{src}$ and a target domain $\mathcal{M}_\textrm{tgt}$, that share the same underlying MDP and task structure (see the graphical model in Figure~\ref{fig:graphicalmodels}) but generate different observations. 
Our key assumption is that in the target domain, the agent only has access to observations \(o_t^\text{tgt}\) and the executed actions \(a_t\), but not the corresponding rewards or the ground-truth state \(s_t\).
% Here, we focus on the case where $\mathcal{M}_\textrm{src}$ and $\mathcal{M}_\textrm{tgt}$ shares the same underlying MDP, while the same state $s_t$ produces vastly different observations $o^\textrm{src}_t$ and $o^\textrm{tgt}_t$ for each domain.
% Often, we are most interested in the case where shift between $\mathcal{M}_\textrm{src}$ and $\mathcal{M}_\textrm{tgt}$ is only induced by differences in the observation spaces $O_\textrm{src}$ and $O_\textrm{tgt}$.
% That is, the state and reward dynamics between the source and target domains are identical, but the observation spaces between the two are significantly different.
A practical example is a robot that is trained with images in a clean, simulated environment that now has to work in-the-wild, in the presence of visual distractors and changes in the lighting condition or the mounting pose of the video camera. These variations could lead to significantly different image observations. As a result of this shift, deploying an agent trained in the source domain directly in the target domain (i.e., zero-shot transfer) generally results in poor performance.

% Given an agent pre-trained on a source domain, our goal is to adapt it to the target domain without relying on either instrumented reward or paired source/target image pairs. %As we do not have knowledge about the correspondence of observations in the two domains, this setting essentially requires us to make use of unpaired trajectory samples from each domain to drive adaptation. 


The proposed method, \lcila, 
%and is pretrained in the source domain $\mathcal{M}_\src$.
aims to adapt the encoder $F$ 
% that maps observations from the source and target domains into a common latent space $Z$ 
in a manner that minimizes distributional shift in $Z$ between the domains. In turn, this enables the policy $\pi_z$ to transfer to the unseen target domain by utilizing only unpaired transitions.
We achieve this by jointly optimizing two objectives: \textit{distribution matching} and \textit{dynamics consistency}.

% Recent work has tried to handle this shift between training and testing environments by greatly expanding the support of the training distribution during training~\citep{sodahansen2020generalization}.\todomw{I added this and the following paragraph from the original submission. We can remove them from this section, but should make sure that the content is somewhere in the paper (probably the intro or related work).} This is most often accomplished via artificial data augmentation. Image observations are cropped, shifted, rotated, and discolored to make learned policies more robust to shifts in the input observation at test time. In RL, this type of augmentation can cause value function estimation to become unstable~\citep{laskin2020reinforcement, Raileanu2020AutomaticDA, Kumar2021regularization}, and so care must be taken to avoid destabilizing training.

% While data augmentation techniques have greatly improved the robustness of RL algorithms to observation shift in the target domain, potential issues linger. %In Figure \ref{fig:tuition}, we see a cartoon illustrating the primary worry. 
% No matter how much the support over the input observation space is expanded, it is common for the size of the target testing observation space to be very small in comparison to the overall size of all observation spaces. Thus, there is still a fairly reasonable chance that even extreme data augmentation measures will fail to adequately cover the target domain's observation space.  Indeed, the results in Section~\ref{sec:experiments} show this to often be the case---even the most robust data augmentation schemes fail when the target observation space differs substantially from that of training. 

% In the next section, we develop a technique, Invariance Through Inference, that enables quick test-time adaptation onto the target observation space by utilizing only unpaired transitions.% without reward. 
% Takuma --- Below is moved to section 4
% The goal of our method is to adapt a feature extractor $F: O \mapsto Z$ that maps observations from the source and target domains into a common latent space $Z$ in a manner that minimizes distributional shift and, in turn, enables the policy to transfer to the unseen target domain. 

% During training, the agent has access to $\mathcal{M}_\textrm{src}$ and can collect trajectory data $\rho_\textrm{src} = (o_i, a_i, r_{i+1}, \ldots)$, where $o_i \in O$, $a_i \in A$, and $r_{i+1} \in R$ is the corresponding reward. % Meanwhile we also train an actor that contains feature extractor $\mathcal{D}_E: o \rightarrow z$ and policy $\pi(a|z)$.
% In the test phase, the agent is placed into the previously unseen $\mathcal{M}_\textrm{tgt}$ environment. Crucially, here we will assume that the agent can only 
% observe a $ (o_\textrm{tgt}, a_\textrm{tgt}) \sim \mathcal{M}_\textrm{tgt}$ i.e., that the agent has no access to the reward function at test time. 
% access observations and actions, but not reward. Our aim is to adapt the feature extractor $\mathcal{D}_E$ by leveraging $\rho_{\text{src}}$ and reward-less trajectories in target domain, so that the policy $\pi(a|z)$ works without any fine-tuning in the unseen target domain.
%
% It should be noted that we do not have access to paired trajectories or observations. Thus this problem can be seen as aligning the latent representations of two domains from unpaired data. 
%
% The proposed method, \iti, achieves this by jointly optimizing two objectives: \textit{distribution matching} and \textit{dynamics consistency}.
% is to leverage the data it collected from $\mathcal{M}_\textrm{src}$, as well as the unsupervised trajectory data $(o_1, a_1, \ldots, o_t, a_t) \sim \mathcal{M}_{tgt}$, and 
%perform fast inference in the target environment:
%
%
% \begin{equation}
%     \mathcal J = \mathbb{E}_{\substack{\rho_\textrm{src} \sim \pi(\mathcal{M}_\textrm{src}) \\ o_{t+1} \sim \pi(o_t, a_t; \rho_\textrm{src})}} \bigg[ r_\textrm{tgt}(o_{t+1}) \bigg],
% \end{equation}
%
%
% where $o_{t+1} \sim \pi(o_t, a_t; \rho_\textrm{train})$  makes clear the dependence of the policy $\pi$ on data from the training environment $\rho_\textrm{train}$. Note that this objective is for evaluation purposes only, because we do not have access to $r_\textrm{test}$ during learning. In the objective, we have used the abuse of notation $o_{t+1} \sim \pi(o_t, a_t; \rho_\textrm{train})$ instead of the correct $o_{t+1} \sim P(o_t, a_t), a_t \sim \pi(o_t; \rho_\textrm{train})$, since the next observation is sampled by following along the policy and space was limited. 

%We will only be able to train by proxy. \\

%\todomw{Why is $o$ drawn from the policy?}

%\todomw{Why is the policy providing a distribution over $o_{t+1}$?}

%\stadie{@Ge Yang, I'd really like to include a figure like Figure 1. Obviously this one sucks. It's worth discussing if we can come up with something that doesn't suck. }

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{illustrations/InvarianceThroughInference.drawio.png}
%     \caption{Expanding the support distribution over the observation space makes the resulting policy much more robust to observation perturbations at test time (Data Augmentation). However, the desired test time observation space is a comparatively small set. No matter how much we expand the support of the input training distribution, there is a chance we will miss the shift captured by the test environment. To avoid this, we consider the problem of how to best carry out additional unsupervised learning at test time.}
%     \label{fig:tuition}
% \end{figure}

%with one crucial change: the agent will not have access to $\mathcal{R}_2$, the reward function for $\mathcal{M}_2$. The agent's goal is to leverage $\mathcal{M}_1$ as effectively as possible to perform better test time inference on $\mathcal{M}_2$ \\

% Takuma -- maybe this is not best fit for problem formulation, maybe should go to intro.
% Often, we are most interested in the case where shift between $\mathcal{M}_\textrm{train}$ and $\mathcal{M}_\textrm{test}$ is induced by differences in the observation spaces $O_\textrm{train}$ and $O_\textrm{test}$. That is, the state and reward structures between the train and test MDPs are quite similar, but the observation spaces between the two MDPs are significantly different. Practically speaking, this can happen quite easily in the presence of distractors, corrupted or malformed inputs, or shifts in sensor readings at test time. Consider a robot that is trained from image observations in a clean environment, and then expected to perform the same task in the wild, where changing lighting conditions and environmental conditions might lead to significantly different image observations. Recent work has tried to handle this shift between training and testing environments by greatly expanding the support of the training distribution during training \citep{sodahansen2020generalization}. This is most often accomplished via artificial data augmentation. Image observations are cropped, shifted, rotated, and discolored to make learned policies more robust to shifts in the input observation at test time. In RL, this type of augmentation can cause value function estimation to become unstable~\citep{laskin2020reinforcement, Raileanu2020AutomaticDA, Kumar2021regularization}, and so care must be taken to avoid destabilizing training.

% Takuma -- maybe this is not best fit for problem formulation, maybe should go to intro.
% While data augmentation techniques have greatly improved the robustness of RL algorithms to observation shift at test time, potential issues linger. In Figure \ref{fig:tuition}, we see a cartoon illustrating the primary worry. No matter how much the support over the input observation space is expanded, the size of the target testing observation space is very small in comparison to the overall size of all observation spaces. Thus, there is still a fairly reasonable chance that even extreme data augmentation measures will fail to adequately cover the test MDP's observation space.  Indeed, the results in Section \ref{sec:experiments} show this to often be the case---even the most robust data augmentation schemes fail when the test MDP's observation space differs substantially from that of training. In the next section, we will develop a technique, Invariance Through Inference, that enables quick test-time adaptation onto the target observation space by utilizing only unsupervised transition pairs. 









% Then talk about SODA and image augmentation, expanding the distribution as wide as possible. 
% Then talk about why that approach will always be insufficient. 

%During testing, the agent will have instead have access to $\mathcal{M}_2$, which can in principle be an entirely different MDP but is nevertheless assumed to share some structure with $\mathcal{M}_1$. The agent's goal is to use  



%our experiments will consider the somewhat restricted setting wherein $\mathcal{M}_1$ and $\mathcal{M_2}$ differ only via their observation spaces $\mathcal{O}_1, \mathcal{O}_2$. 

% There are actually two MDPs, one on train and one on test. 
% The goal of methods like SODA is to expand the support distribution during the train phase, so that there's a higher chance it overlaps with the test distribution. 
% Maybe try and make a graphic that conveys this point. 
% PAD, train on test have this idea of instead training directly on the test distribution. We want 

%thus, we want a method that uses training to greatly accelerate test time inference. 

%\subsection{Problem Formulation}



==> sections/related_work.tex <==
\section{Related Work}

A large body of work is dedicated to improving the ability for neural networks to generalize.  These works can largely be put into two categories -- the first category, including domain randomization, data augmentation, empirical risk minimization, and meta-learning, all make the assumption that one has a rough idea of what type of perceptual change occurs during deployment. In meta-learning the key assumption is one has access to a meta-distribution of task/environment pairs. This is an even stronger assumption than those typically made by supervised learning, that the data is sampled from an i.i.d that covers the test distribution. In many cases especially in reinforcement learning, generalization comes from the exposure to a large amount of diverse data. Meta learning offers very little gain procedural-wise, because a meta-learning algorithm is externally identical to multi-task training, except that the higher-order gradients are limited in expressivity, and more complex to compute.

The second category of methods, which this proposal is also a member of, makes no explicit assumption of what type of distribution shift occurs in the target domain. They include approaches such as unsupervised domain adaptation, train-on-test, and \textit{tailoring}. These methods all approach adaptation as an out-of-distribution generalization problem where what happens in the target domain can not be known when training the model. These approaches differentiate the testing phase from the training phase by what types of information is privileged, therefore only available during training. Some examples include ground-truth labels under supervised learning, segmentation masks for dense predictions in computer vision, or instrumented rewards during reinforcement learning. Without these privileged information available at test time, these approaches all cast adaptation as an unsupervised, or self-supervised learning process, with main difference being the learning objective, optimization details, and ways to augment the data. In particular, test-time adaptation by entropy minimization~\cite{wang2020tent} shows that fine-tuning just the two parameters in layernorm gives better performance than fine-tuning the entire network. CycADA and FCN in the wild uses cycle-consistent, adversarial loss for matching pixel-wise dense features~\cite{Hoffman2017cycada,Hoffman2016wild}. Some of these methods~\cite{Sankaranarayanan2017synthetic} produce feature alignment by synthesizing image pixels, whereas our proposal only enforces alignment in the latent space using an adversarial objective.

% Instead, they make the distinction that the test-time differs from training time in that categories of \textit{privilleged information}, such as labels under supervised learning, or rewards in learning to control, 
% Meta-learning
% Unsupervised Domain adaptation
% Learning symmetries

\todoty{I have in mind what each citation refers to. I just haven't filled it yet}
%\stadie{First draft done. Ready for input from other authors (Ge, Takuma, Matt) -- Oct 1 at 17:20.  }
\textbf{Expanding the training distribution} helps a model to generalize to a new domain within the support of the distribution. One approach in this family is \textit{data augmentation} which has been successfully used in computer vision community \citep{}. In the similar way, pixel-based RL also benefitted from it \citep{}. % Quantifying generalization in reinforcement learning, A simple technique for generalization in deep reinforcement learning.
More recently, several papers pointed out that naive data augmentation causes instability in value function estimation, and showed how to stabilize the training \citep{}. % RAD, DrQ, DrQv2, SODA, SVEA
Another approach is \textit{domain randomization} which randomly modifies the environment at every episode, thereby exposing the agent to a wider training distribution. This approach has been extensively applied especially in the context of sim-to-real transfer \citep{}. % Four papers here

\textbf{Unsupervised Domain Adaptation} considers a pair of source and target domain, where supervision (e.g., labeled data) is only available in the the source domain. After training a model in source domain, the task is to adapt it such that it can achieve a small test error in the target domain.
A common approach is to train a network such that it minimizes a task loss while maximizing domain confusion loss \citep{}. This encourages the latent representation to be domain-invariant. This idea has been applied successfully in imitation learning \citep{stadie2017third}. Employing the adversarial loss in generative adversarial networks (GANs) \citep{goodfellow2016nips} rather than the original mini-max objective has shown even better performance \citep{}. % ADDA, Unsupervised Pixel-level DA, CyCADA
There are a few method for RL that employs GAN in the same way \citep{}. Our method also falls into this category. Among these methods, \citep{} is the closest to our approach. The key differences are (1) they train encoder only from reconstruction and latent dynamics, without utilizing the available reward signals; and (2) they experiment the method on a single toy environment.

% \textbf{Generalization in reinforcement learning} is a longstanding problem~\cite{tan18}. % \todomw{Not the best place for this reference, but it wasn't obvious where else to put it}
% Recent work has shown that accurately quantifying generalization in this setting poses a challenge~\citep{Lee2019ASR, cobbe2018quantifying, zhang2018dissection}. This challenge is further amplified in visual RL from pixels, where measuring the difference between two problems is especially difficult. One promising class of techniques for generalization in image-based RL utilize image augmentation to greatly increase the size of the training distribution. These techniques have enjoyed success in vision research~\citep{chen2020simple, He2020MomentumCF}. However, it was only recently shown that such data augmentation leads to instability in value function estimation in RL algorithms~\citep{sodahansen2020generalization, svea}. This line of work as well as \citep{active-domain-randomization} showed how to stabilize data-augmented RL, which lead to a significant increase in the generalization capabilities of RL algorithms. The primary shortcoming of these methods is that it is largely impossible to effectively cover the entire potential test distribution by expanding the training distribution, and some test time adaptation is often needed. Several recent works~\citep{padhansen2020selfp, wang2020tent} % \todomw{We should expand on the discussion of \cite{zhang2021policy} since it is (a) relevant and (b) was published at RSS}
% consider this setting of adaptation at test time. % , and are further discussed in Section \ref{sec:problem}.

% \textbf{Invariant Representation Learning} is a broad class of techniques for learning representations that are robust across changes in the agent's environment or reward. Often, the agent will use auxiliary information related to dynamics~\citep{hafner2020mastering} or reward prediction~\citep{jaderberg2016reinforcement} to learn a latent representation that is invariant across changing environmental conditions. This is closely related to the idea of \textbf{self-supervised learning}~\citep{Chen2020AdversarialFT, Grill2020BootstrapYO}. When applied to visual space RL, it has been shown that self-supervised pre-training provides an efficient way to bootstrap useful invariant representations, even in the absence of a ground-truth reward~\citep{schwarzer2020data, srinivas2020curl}. 
% Another class of approach is to learn representations that maximize domain confusion, thus requiring that the agent learn domain-invariant features. This idea has been applied successfully in imitation learning~\citep{stadie2017third}. More recent advances have combined Cycle-GANs with imitation learning to produce features that are cycle consistent across domains~\citep{smith2019avid}. Another approach bottlenecks the information on the latent code of a VAE-based architecture to learn features that are more robust across domain shift in a variety of adversarial settings~\citep{Peng_2018}. Some other works focus on the domain shift in dynamics properties, and learn action transformation to align the transition between domains~\citep{AAAI17-Hanna, garat2020}. There is also an attempt to deal with both observation and dynamics domain shift by combining these ideas~\citep{zhang2021policy}.
% List of papers to include:
% - Unsupervised Visual Attention and Invariance for Reinforcement Learning
% A new family of approach to decouple representation learning
% - Decoupling Representation Learning from Reinforcement Learning

% \textbf{Unsupervised Domain Adaptation} considers a pair of source and target domains, where labeled data or reward is only available in the source domain. We can train a model in source domain with supervision, and the task here is to adapt the model to the target domain in some way. In the context of RL,...
% This problem has been discussed even without the context of RL 
% ^ If we begin to talk about unsupervised domain adaptation in general, we need to mention hundreds of papers.

% List of papers to include
% - Cycada: Cycle-Consistent Adversarial Domain Adaptation
% - Adversarial Discriminative Sim-to-real Transfer of Visuo-motor Policies

% \textbf{Domain Shift} considers the problem of test-time shift in the underlying input data distribution~\citep{ganin2016domain, Hoffman_cycada2017}. One common class of techniques for addressing this problem is to learn representations that maximize domain confusion, thus requiring that the agent learn domain-invariant features. This idea has been applied successfully in imitation learning~\citep{stadie2017third}. More recent advances have combined Cycle-GANs with imitation learning to produce features that are cycle consistent across domains~\citep{smith2019avid}. Another approach bottlenecks the information on the latent code of a VAE-based architecture to learn features that are more robust across domain shift in a variety of adversarial settings~\citep{Peng_2018}. Some other works focus on the domain shift in dynamics properties, and learn action transformation to align the transition between domains~\citep{AAAI17-Hanna, garat2020}. There is also an attempt to deal with both observation and dynamics domain shift by combining these ideas~\citep{zhang2021policy}.
\todoty{This should also fit in "Expanding the training distribution"}
\textbf{Meta Learning} tries to solve generalization by aggregating learning across distributions of tasks~\citep{maml, rl2, pearl}. Often, meta learning pipelines focus heavily on fast inference at test time. This is most often accomplished through using some form of bi-level optimization~\citep{promp, epg}. Unfortunately, meta learning methods generally require training over entire task distributions. Worse still, this results in the need for a distribution of reward functions for each task during both training and test time. Defining even a single reward function is often quite difficult, let alone many closely related reward functions. Recent work has tried to alleviate this burden with unsupervised training~\citep{cactushsu2018unsupervised}. 

%, wherein it has recently been shown that vision pipelines for RL tasks can learn more efficiently and with lower error when combined with self-supervised pre-training. 







%Cycle Gan for third person imitation.   


%Imitation learning (third person), RL (changing lighting conditions) here. Also talk about the problem more generally. 







%\cite{yarats2019improving} is cool

%Meta learning -- requires a wide distribution of tasks 

%Expanding the distribution -- SODA, VERA 

%Train on test -- PAD, (tent)



%\paragraph{train-on-test literature: tent, PAD}, + (not train on test but pre-baked in) SODA, VERA 
%\paragraph{cycle GAN literature}
%\paragraph{imitation and IRL literature}
%\paragraph{information bottleneck (Jason Peng)}
%\paragraph{Domain Shift, Meta Learning, Third Person Imitation Learning}g
